The Sample-Communication Complexity Trade-off in Federated Q-Learning

We consider the problem of federated Q-learning, where $M$ agents aim to collaboratively learn the optimal Q-function of an unknown infinite-horizon Markov decision process with finite state and action spaces. We investigate the trade-off between sample and communication complexities for the widely used class of intermittent communication algorithms. We first establish the converse result, where it is shown that a federated Q-learning algorithm that offers any speedup with respect to the number of agents in the per-agent sample complexity needs to incur a communication cost of at least an order of $\frac{1}{1-\gamma}$ up to logarithmic factors, where $\gamma$ is the discount factor. We also propose a new algorithm, called Fed-DVR-Q, which is the first federated Q-learning algorithm to simultaneously achieve order-optimal sample and communication complexities. Thus, together these results provide a complete characterization of the sample-communication complexity trade-off in federated Q-learning.

==> achievability.tex <==
\section{Trading off Sample and Communication Complexities}

In the previous section, we described the \DVR algorithm that established achievability of a single sample-communication pair on the trade-off curve. In this section, we describe the $\alpha$-\DVR~algorithm, that consists of a tunable parameter $\alpha \in (0,1)$. For a given target accuracy $\varepsilon$, $\alpha$-\DVR allows the learner to trade-off communication complexity for sample complexity based on the choice of $\alpha$, while maintaining the required target accuracy $\varepsilon$. Thus, $\alpha$-\DVR traces out the achievability frontier of the sample-communication complexity trade-off curve. \\

% \red{Wanted your opinion on this section. My basic idea was to use different mean estimation routine to allow for smaller communication costs each round at the price of increased sample complexity. This shows that the trade-off is linear and how one can achieve the entire optimal front. If you think it is worth adding and discussing, I will add the details about this variant here.}



% In the previous section, we described the \DVR algorithm that established achievability of a single sample-communication pair on the optimal frontier. In this section, we describe the $\alpha$-\DVR algorithm, that 
% can be made to operate at any desired point on the frontier by appropriately tuning the parameter $\alpha \in (0,1)$. The core idea of $\alpha$-\DVR is to combine \DVR with partial participation of clients in such a way that it allows $\alpha$-\DVR to trade-off sample complexity for communication complexity along the optimal frontier.

There are three main differences $\alpha$-\DVR and \DVR. Firstly, $\alpha$-\DVR consists of a tunable parameter $\alpha \in (0,1)$ that controls the trade-off between sample and communication complexity. Secondly, the compressor $\sC$ sends the value of only $\lceil \alpha |\cS| |\cA| \rceil$ coordinates of the input vector, which are chosen uniformly at random and are independent from the previous calls to the compressor. Lastly, the parameters $B$ and $N_k$ used in $\alpha$-\DVR are set to
\begin{align}
    B= \left\lceil \frac{2}{M}\left(\frac{12\gamma}{(1-\gamma)}\right)^2  \log\left(\frac{8KL|\cS||\cA|}{\delta} \right) \right\rceil; \quad N_k  :=  \frac{19600}{\alpha(1-\gamma)^2} \log\left(\frac{8KL|\cS||\cA|}{\delta} \right) \cdot\begin{cases} 4^k & \text{ if } k \leq K_0 \\ 4^{k-K_0} & \text{ if } k > K_0 \end{cases}, 
\end{align}
while all the others are kept the same as \DVR. The increased batch size results in an increased sample complexity. However, since only $\alpha$ fraction of coordinates are transmitted in each round, the communication complexity reduces by a factor of $\alpha$. The following theorem characterizes the sample and communication complexities of $\alpha$-\DVR.



% for each iteration $l$ of \RE, the server chooses a set of $\lceil \alpha M \rceil$ agents uniformly at random, denoted by $\cD_l$, independent of other iterations. During the $l^{\text{th}}$ iteration, only the agents in the set $\cD_l$ participate in updating the value $Q_{l-1}^{(m)}$. Lastly, the selected agents $\cD_l$ use a larger batch size of $B/\alpha = \cO(\frac{1}{\alpha(1-\gamma)^{2}})$ to ensure the same level of progress as \DVR in each iteration. The increased batch size results in an increased sample complexity. However, since each agent participates only $\alpha$ fraction of the time, the communication complexity reduces by a factor of $\alpha$

% \begin{theorem}
%     Consider any given $\delta \in (0,1)$ and $\varepsilon \in (0, \frac{1}{1-\gamma}]$. Under the federated learning setting described in Section~\ref{}, the sample and communication complexities of the $\alpha$-\DVR algorithm, when run with the choice of parameters described in Sec.~\ref{}, a learning rate $\eta \in (0,1)$ and any choice of $\alpha \in (1/M,1)$, satisfy the following relations:
%     \begin{align}
%         \cN(\alpha\textsf{-Fed-DVR-Q }; \varepsilon, \delta) \leq  \\
%         \cC(\alpha-\DVR; \varepsilon, \delta) \leq.
%     \end{align}
% \end{theorem}

% Thus, partial participation allows $\alpha$-\DVR to achieve a smaller communication complexity at the cost of higher sample complexity. Moreover, the product of sample and communication complexities of $\alpha$-\DVR match the lower bound (upto logarithmic factors) for all values of $\alpha$, thereby ensuring it always operates on the optimal frontier of the sample-communication complexity trade-off.

==> lower_bound_proof.tex <==
\section{Proof of General Lower Bound}

% \begin{assumption}
%     Stochastic Oracle: Unbiased, $\sigma$^2-sub-Gaussian
% \end{assumption}

% \begin{assumption}
%     $\cT : \cX \to \cX$ is $\gamma$-contractive in $\ell_{\infty}$ norm, i.e., for any $x_1, x_2 \in \cX$, $\|\cT(\bfx_1) - \cT(\bfx_2)\|_{\infty} \leq \gamma \|\bfx_1 - \bfx_2\|_{\infty}$
% \end{assumption}

% WLOG, we assume that $\bfzero \in \cX$. For simplicity, we assume $\cX = \R^d$, however, it can be any compact subset of $\R^d$.

% \begin{assumption}
%     The distributed mean estimation routine $\textsc{Mean}(X)$, returns an estimate $\hat{X}$ such that $\E[\hat{X}] = X$ and $\hat{X} - X$ is $\sigma_{\mean}^2$-sub-Gaussian.
% \end{assumption}

In order to establish the lower bound, we first consider an operator in $\R^3$ and establish the lower bound over $\R^3$. In Sec.~\ref{}, we generalize our construction of the ``hard'' instance to higher dimensional spaces and extend our insights to obtain the statement of the theorem. \\


Consider the following operator $\cT: \R^3 \to \R^3$ for $\gamma \in (0,1)$.
\begin{align*}
    \cT(\bfx) =  \begin{bmatrix} \gamma\max\{\bfx(1), \bfx(2)\} \\ \gamma\max\{\bfx(1), \bfx(2)\} \\ \gamma\bfx(3) + (1-\gamma)\sigma  \end{bmatrix}.
\end{align*}
It is straightforward to note that the operator $\cT$ satisfies $\|\cT(\bfx) - \cT(\bfy)\| \leq \gamma \|\bfx - \bfy\|_{\infty}$ for all $\bfx, \bfy \in \R^3$. Moreover, $\bfx^{\star} = (0,0,\sigma)^{\top}$ is the unique fixed point of the operator. We consider a stochastic oracle of the form
\begin{align}
    \hat{\cT}(\bfx) = \cT(\bfx) + \bfz,
\end{align}
where $\bfz = [\bfz(1), \bfz(2), \bfz(3)]^{\top}$ and $\bfz_(i)$ are i.i.d. variables for all $i = 1,2,3$ and take the values $\{-\sigma, \sigma\}$ with probability $1/2$. It can be verified that $\hatT$ satisfies Assumption~\ref{ass:operator_noise}.
%WLOG, we assume $\sigma \leq D$. If $\sigma > D$, then we can replace $\sigma$ with $\min\{\sigma, D\}$. 
Let $\widehat{\bfz} \sim \frac{1}{B} \sum_{b = 1}^B \bfz_b$, where $\bfz_b$ are i.i.d. random variables distributed as $\bfz$. We use $\widehat{\bfz}$ to denote the noise in the algorithm in case of minibatching with $B$ samples.

\subsubsection{Notation}

For convenience, we first define some notation that we will use throughout the proof. We consider two kinds of step size sequences that are commonly used in stochastic fixed point iterations --- the constant step size, i.e., $\eta_t = \eta$ for all $t \in \{1,2,\dots, T\}$ and the rescaled linear step size schedule, i.e., $\eta_t = \frac{1}{1 + c_{\eta}(1-\gamma)t}$, where $c_\eta > 0$ is constant. \\

We define the following quantities:
\begin{align}
    \eta_k^{(t)} & = \eta_k \prod_{i = k+1}^t (1- \eta_i(1- \gamma)) ~~~~~~~~~ \text{ for all } 0 \leq k \leq t, \label{eqn:eta_k_t_defn} %\\
    % \eta_0^{(t)} & = \prod_{i = 1}^t (1- \eta_i(1- \gamma p)) \\
    % \eta_t^{(t)} & = \eta_t.
\end{align}
where we take $\eta_0 = 1$ and use the convention that if a product operation does not have a valid index, we take the value of that product to be $1$. Throughout the proof, we adopt the above convention regarding product operations. For any integer $0 \leq \tau < t$, we have the following relation:
\begin{align}
    \prod_{k = \tau + 1}^t (1- \eta_k(1-\gamma)) + (1- \gamma) \sum_{k = \tau + 1}^t \eta_k^{(t)} = 1. \label{eqn:eta_k_t_recursion}
\end{align}
We can show the claim using backward induction. For the base case, note that,
\begin{align*}
    (1-\gamma)\eta_t^{(t)} + (1-\gamma)\eta_{t-1}^{(t)} & = (1- \gamma)\eta_t + (1-\gamma)\eta_{t-1}(1 - (1- \gamma)\eta_t) \\
    & = 1 - (1- \eta_t(1-\gamma))(1-\eta_{t-1}(1 -\gamma)) = 1 - \prod_{k = t-1}^t (1- \eta_k(1-\gamma)),
\end{align*}
as required. Assume true for some $\tau$. We have,
\begin{align*}
    (1- \gamma ) \sum_{k = \tau }^t \eta_k^{(t)} & = (1- \gamma)\eta_{\tau}^t + (1- \gamma) \sum_{k = \tau + 1}^t \eta_k^{(t)} \\
    & = (1-\gamma )\eta_{\tau}\prod_{k = \tau + 1}^t (1- \eta_k(1-\gamma ))  + 1 - \prod_{k = \tau + 1}^t (1- \eta_k(1-\gamma )) \\
    & = 1 - \prod_{k = \tau}^t (1- \eta_k(1-\gamma )),
\end{align*}
completing the inductive step. Similarly, we also define,
\begin{align}
    \widetilde{\eta}_k^{(t)} & = \eta_k \prod_{i = k+1}^t (1- \eta_i) ~~~~~~~~~ \text{ for all } 0 \leq k \leq t, \label{eqn:tilde_eta_k_t_defn} %\\
    % \eta_0^{(t)} & = \prod_{i = 1}^t (1- \eta_i(1- \gamma p)) \\
    % \eta_t^{(t)} & = \eta_t.
\end{align}
which satisfies the relation 
\begin{align}
    \prod_{k = \tau + 1}^t (1- \eta_k) + \sum_{k = \tau + 1}^t \widetilde{\eta}_k^{(t)} = 1. \label{eqn:tilde_eta_k_t_recursion}
\end{align}
for any integer $0 \leq \tau < t$. The claim follows immediately by plugging $\gamma = 0$ in Eqn.~\eqref{eqn:eta_k_t_recursion}. Note that for constant step size, the sequence $\widetilde{\eta}_k^{(t)}$ is clearly increasing. For the rescaled linear step size, we have, 
\begin{align}
    \frac{\widetilde{\eta}_{k-1}^{(t)}}{\widetilde{\eta}_{k}^{(t)}} = \frac{\eta_k}{\eta_{k-1}(1-\eta_k)} = 1- \frac{(1 - c_{\eta}(1-\gamma))\eta_k}{1 - c_{\eta}(1 - \gamma)\eta_k} \leq 1,\label{eqn:tilde_eta_k_t_increasing}
\end{align}
whenever $c_{\eta} \leq \frac{1}{1 - \gamma}$. Thus, $\widetilde{\eta}_k^{(t)}$ is an increasing sequence as long as $c_{\eta} \leq \frac{1}{1 - \gamma}$. For any $t', t$ with $t' < t$, we define,
\begin{align}
    \varphi_{t', t} := \prod_{k = t' + 1}^t (1- \eta_k) \label{eqn:varphi_defn}
\end{align}

For the remainder of the proof, we define 
\begin{align}
    \tau := \min \{ k \in \N : \forall \ t \geq k, \eta_t \leq \eta_{k} \leq 2 \eta_{t} \}. \label{eqn:tau_def}
\end{align}
It can be noted that for constant step size sequence $\tau = 1$ and for rescaled linear stepsize $\tau = T/2$. Moreover, we assume that $T \geq 3$ and $\log T \leq \log \left( \frac{1}{1- \gamma} \right) + \frac{1}{2(1-\gamma)}$. Lastly, throughout the analysis, we assume that the algorithm is run with a batch size of $B' = \max\{B, 130\}$ and total sample complexity of the algorithm is lower bounded as  $N = BT \geq B'T/130$. Having a lower bound on the batch size only helps reduces noise and improves the convergence guarantee of the original algorithm. The rationale for having a minimum batch size is purely for analytical convenience and only affects the leading constant in the lower bound.

\subsubsection{Small Learning Rates}

In this subsection, we prove the lower bound for small learning rates. Throughout the section, we assume that for constant learning rates, $0 \leq \eta < \frac{1}{(1- \gamma)T}$ and for rescaled linear learning rates, the constant $c_{\eta}$ satisfies $c_{\eta} \geq \log T$. \\

For this case, we focus on the dynamics of the third coordinate. From the definition of our operator $\cT$, it is straightforward to note that the evolution of the third coordinate is independent of the other coordinates. This yields the following recursive relation for $\bfx_t(3)$.
\begin{align*}
    \bfx_{t-1/2}^m(3) & = (1 - \eta_t)\bfx_{t-1}^m(3) + \eta_t \gamma \bfx_{t-1}^m(3) + \eta_t(1-\gamma)\sigma + \eta_t \hatbfz_t^m \\
    & = (1 - \eta_t(1-\gamma))\bfx_{t-1}^m(3) + \eta_t(1-\gamma)\sigma + \eta_t \hatbfz_t^m \\
\end{align*}
When $t$ is not an averaging instant, we have,
\begin{align}
    \bfx_{t}^m(3) & = (1 - \eta_t(1-\gamma))\bfx_{t-1}^m(3) + \eta_t(1-\gamma)\sigma + \eta_t \hatbfz_t^m \nonumber \\
    \implies \E[\bfx_{t}^m(3)] & = (1 - \eta_t(1-\gamma))\E[\bfx_{t-1}^m(3)] + \eta_t(1-\gamma)\sigma. ~\label{eqn:coord_3_update_case_1}
\end{align} 
Similarly, if $t$ is an averaging instant, we have,
\begin{align}
    \bfx_{t}^m(3) & = \frac{(1 - \eta_t(1-\gamma))}{M}\sum_{j = 1}^M \bfx_{t-1}^j(3) + \eta_t(1-\gamma)\sigma + \frac{\eta_t}{M} \sum_{j = 1}^M \hatbfz_t^j \nonumber \\
    \implies \E[\bfx_{t}^m(3)] & = (1 - \eta_t(1-\gamma)) \left(\frac{1}{M} \sum_{j = 1}^M \E[\bfx_{t-1}^j(3)] \right) + \eta_t(1-\gamma)\sigma. ~\label{eqn:coord_3_update_case_2}
\end{align} 
Eqns.~\eqref{eqn:state_2_value_update_case_1} and~\eqref{eqn:state_2_value_update_case_2} together imply that for all $t \in [T]$, 
\begin{align}
    \left(\frac{1}{M} \sum_{m = 1}^M  \E[\bfx_{t}^m(3)]\right) = (1 - \eta_t(1-\gamma)) \left(\frac{1}{M} \sum_{j = 1}^M \E[\bfx_{t-1}^j(3)] \right) + \eta_t(1-\gamma)\sigma.
\end{align}
On unrolling the above recursion with $\bfx_0^m(3) = 0$ for all $m \in [M]$, we obtain,
\begin{align}
    \E[\bfx_T^m(3)] = \left(\frac{1}{M} \sum_{j = 1}^M  \E[\bfx_T^m(3)]\right) = (1-\gamma)\sigma\sum_{k = 1}^T \eta_k^{(t)} =  \sigma(1 - \eta_0^{(T)}).
\end{align}
Consequently, for all $m \in [M]$, we have
\begin{align*}
    \E[|\bfx^{\star}(3) - \bfx_T^m(3)|] \geq |\sigma - \E[\bfx_T^m(3)]| \geq \sigma \eta_0^{(T)}.
\end{align*}
To obtain lower bound on $\E[|\bfx^{\star}(3) - \bfx_T^m(3)|]$, we need to obtain a lower bound on $\eta_0^{(T)}$. To that effect note that for any step size schedule of our choice,
\begin{align*}
    \eta_t(1- \gamma) \leq (1-\gamma) \max\left\{ \frac{1}{(1- \gamma)T}, \frac{1}{1 + \log T(1-\gamma)t}\right\} \leq \frac{1}{2}, 
\end{align*}
as $T \geq 3$. Consequently, 
\begin{align*}
    \log(\eta_0^{(T)}) & \geq \sum_{t = 1}^T \log(1 - \eta_t(1- \gamma)) \geq -1.5\sum_{t = 1}^T \eta_t(1- \gamma).
\end{align*}
For constant step size, we have,
\begin{align*}
    \log(\eta_0^{(T)}) \geq -1.5\sum_{t = 1}^T \eta(1- \gamma) \geq -2\sum_{t = 1}^T \frac{1}{T} \geq -2.
\end{align*}
Similarly for rescaled linear step size,
\begin{align*}
    \log(\eta_0^{(T)}) \geq -1.5\sum_{t = 1}^T \eta(1- \gamma) \geq -2\sum_{t = 1}^T \frac{1}{t \log T} \geq -2.
\end{align*}
Hence, for both the cases, $\eta_0^{(T)} \geq e^{-2}$. Thus, for all $m \in [M]$,
\begin{align}
    \ER(\sA; N, M) = \E[\|\bfx_T^m - \bfx_{\star}\|_{\infty}] \geq \E[|\bfx^{\star}(3) - \bfx_T^m(3)|] \geq \frac{\sigma}{e^2} \geq \frac{\sigma}{e^2 \sqrt{N}}. \label{eqn:err_small_lr_final_bound}
\end{align}
Thus, it can be noted that the error rate is bounded away from a constant value irrespective of the number of agents and the number of communication rounds. Thus, even with $\CC_{\textsf{round}} = \Omega(T)$, the error rate will not decrease as a the number of agents increase if the step size is too small.

\subsubsection{Large Learning Rates}

In this subsection, we prove the lower bound for large learning rates. Throughout the section, we assume that for constant learning rates, $\eta \geq \frac{1}{(1- \gamma)T}$ and for rescaled linear learning rates, the constant $c_{\eta}$ satisfies $0 \leq c_{\eta} \leq \log T$. For the analysis with large learning rates, we focus on the evolution of the first and the second coordinates. 
% Moreover, since quantization makes the learning problem harder, we assume that the distributed mean estimation routine returns the exact mean with no quantization error. 
We first focus on bounding the communication cost only in terms of frequency and we will bound the bit level cost separately. \\

Note that since $\bfx^{\star}(1) = \bfx^{\star}(2) = 0$, the error $\bfx_t(i) - \bfx^{\star}(i)$ depends only on $\bfx_t(i)$ for $i = 1,2$. Thus, we focus on bounding the value of $\bfx_t(i)$ for $i =1,2$ across iterations. To that effect, we define the following for all $t \leq T$ and all $m \in [M]$: 
\begin{align*}
    x_{t, \max}^m & = \max_{i \in \{1,2\}} \bfx_t^m(i).
\end{align*}
From the iterative update rule from Alg.~\ref{alg:general_fed_alg_with_inter_comm}, the following relation holds for $i = 1,2$:
\begin{align*}
    \bfx_{t-1/2}^{m}(i) & = (1 -\eta_t)\bfx_{t-1}^m(i) + \eta_t \gamma \max\{|\bfx_{t-1}^m(1)|, |\bfx_{t-1}^m(2)|\} + \eta_t \hatbfz_t^m(i). \\
    % & \geq (1 -\eta_t)\bfx_{t-1}^m(i) + \eta_t \gamma \bfx_{t, \max}^m  + \eta_t \bfz_t^m(i).
\end{align*}
We can recursively unroll this expression to obtain the following relation for any $t' < t$ assuming that there is no averaging during the interval $(t',t)$.
\begin{align}
    \bfx_{t}^{m}(i)  & = \left(\prod_{k = t' +1}^t (1- \eta_k) \right) \bfx_{t'}^{m}(i)  +  \sum_{k = t' + 1}^t \left( \eta_k  \prod_{i = k+1}^t (1- \eta_i) \right) (\gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\} + \hatbfz_t^m(i)) \nonumber \\
    & = \varphi_{t', t} \bfx_{t'}^{m}(i)  +  \sum_{k = t' + 1}^t \widetilde{\eta}_k^{(t)} (\gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\} + \hatbfz_t^m(i)). \label{eqn:delta_t_recursive_eqn_orig}
\end{align}
Let
\begin{align}
    \xi_{t', t}^m(i) & := \sum_{k = t' + 1}^t \widetilde{\eta}_k^{(t)} \hatbfz_k^m(i) , \quad i = 1,2; \label{eqn:xi_def} \\
    \xi_{t', t, \max}^m & := \max_{i \in \{1,2\}} \xi_{t', t}^{m}(i). \label{eqn:xi_max_def}
\end{align}
Note that by definition, $\E[\xi_{t',t}^m(i)] = 0$ for $i \in \{1,2\}$ and all $m$, $t'$ and $t$. Then, we can rewrite the Eqn.~\eqref{eqn:delta_t_recursive_eqn_orig} as
\begin{align*}
    \bfx_{t}^{m}(i) & =  \varphi_{t', t} \bfx_{t'}^{m}(i) +  \left[\sum_{k = t' + 1}^t \widetilde{\eta}_k^{(t)} \gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\} \right] + \xi_{t',t}^m(i).
\end{align*}
We specifically choose $t'$ and $t$ to be the consecutive averaging instants to analyze the behaviour of $\bfx_t^m$ across two averaging instants. For clarity of notation, we use $\barbfx$ to denote the error of the averaged iterate and $\bfx$ to denote the error before averaging (as opposed to using the half time indices). Consequently, we can rewrite the above equation as
\begin{align}
    \bfx_{t}^{m}(i) & =   \varphi_{t', t} \barbfx_{t'}^{m}(i) +  \left[\sum_{k = t' + 1}^t \widetilde{\eta}_k^{(t)} \gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\}\right] + \xi_{t',t}^m(i). \label{eqn:delta_m_unaveraged}
\end{align}
Furthermore, after averaging, we obtain,
\begin{align}
    \barbfx_{t}^{m}(i) & =  \varphi_{t', t} \barbfx_{t'}^{m}(i) +  \frac{1}{M} \sum_{m = 1}^M \left[\sum_{k = t' + 1}^t  \lambda_{k, t} \gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\} \right] + \frac{1}{M} \sum_{m = 1}^M \xi_{t',t}^m(i)  \label{eqn:delta_m_averaged} %+ \frac{1}{M} \sum_{m = 1}^M \zeta_{t, \quant}^m(i),
\end{align}
% where $\zeta_{t, \quant}^m(i)$ denotes the zero-mean quantization noise introduced by the mean estimation routine. 
Using Eqn.~\eqref{eqn:delta_m_unaveraged}, we obtain,
\begin{align}
    x_{t, \max}^m & \geq \varphi_{t', t}  \barx_{t', \max} +  \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\}  \right] + \xi_{t',t, \max}^m - \varphi_{t', t} |\barbfx_{t'}(1) - \barbfx_{t'}(2)| \label{eqn:delta_max_unaveraged_lower_bound} \\
    x_{t, \max}^m & \leq \varphi_{t', t}  \barx_{t', \max} +  \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\}  \right] + \xi_{t',t, \max}^m   \label{eqn:delta_max_unaveraged_upper_bound}
    % \implies \E[\bfx_{t, \max}^m] & \geq \varphi_{t', t}  \E[\barbfx_{t', \max}] +  \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma p\E[\bfx_{k-1, \max}^m] \right] + \E[\xi_{t',t, \max}^m] - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|], \label{eqn:delta_max_unaveraged_expectation}
\end{align}
where in the first step we used the fact that
\begin{align}
    \max\{a_1 + b_1, a_2 + b_2\} \geq \min\{a_1, a_2\} + \max\{b_1, b_2\} = \max\{a_1, a_2\} + \max\{b_1, b_2\} - |a_1 - a_2|. \label{eqn:max_decomposition}
\end{align}
On taking expectation, we obtain,
\begin{align}
    \E[x_{t, \max}^m] & \geq \varphi_{t', t}  \E[\barx_{t', \max}] +  \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \E[\max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\}]  \right] + \E[\xi_{t',t, \max}^m] - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|] \label{eqn:delta_max_unaveraged_expectation_lower_bound} \\
    \E[x_{t, \max}^m] & \leq \varphi_{t', t}  \E[\barx_{t', \max}] +  \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \E[\max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\}]  \right] + \E[\xi_{t',t, \max}^m].   \label{eqn:delta_max_unaveraged_expectation_upper_bound}
\end{align}
Similarly, using Eqn.~\eqref{eqn:delta_m_averaged} and~\eqref{eqn:max_decomposition} we can write,
\begin{align}
    \barx_{t, \max} & \geq \varphi_{t', t}  \barx_{t', \max} +  \frac{1}{M} \sum_{m = 1}^M \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\} \right] - \varphi_{t', t} |\barbfx_{t'}(1) - \barbfx_{t'}(2)|   \nonumber \\
    & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ + \max\left\{ \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(1) , \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(2) \right\}  \label{eqn:delta_max_averaged} \\ %+ \max\left\{ \frac{1}{M}\sum_{m = 1}^M (\xi_{t',t}^m(1) + \zeta_{t, \quant}^m(1)), \frac{1}{M}\sum_{m = 1}^M (\xi_{t',t}^m(2) + \zeta_{t, \quant}^m(2)) \right\}
    \implies \E[\barx_{t, \max}] & \geq \varphi_{t', t}  \E[\barx_{t', \max}] + \frac{1}{M} \sum_{m = 1}^M \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \E[\max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\}] \right] - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|] \nonumber  \\
    & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ + \E\left[\max\left\{ \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(1), \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(2)  \right\}\right], \label{eqn:delta_max_averaged_expectation} %+ \max\left\{ \frac{1}{M}\sum_{m = 1}^M (\xi_{t',t}^m(1) + \zeta_{t, \quant}^m(1)), \frac{1}{M}\sum_{m = 1}^M (\xi_{t',t}^m(2) + \zeta_{t, \quant}^m(2)) \right\}
\end{align}
% where we once again used Eqn.~\eqref{eqn:max_decomposition}.
On combining Eqns.~\eqref{eqn:delta_max_unaveraged_expectation_upper_bound} and~\eqref{eqn:delta_max_averaged_expectation}, we obtain,
\begin{align}
    \E[\barx_{t, \max}] & \geq \frac{1}{M} \sum_{m = 1}^M \left[\E[x_{t, \max}^m] - \E[\xi_{t',t, \max}^m]\right] - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|]  + \E\left[\max\left\{ \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(1), \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(2) \right\}\right]. \label{eqn:barDelta_max_as_func_clients} %\E\left[\max\left\{ \frac{1}{M}\sum_{m = 1}^M (\xi_{t',t}^m(1) + \zeta_{t, \quant}^m(1)), \frac{1}{M}\sum_{m = 1}^M (\xi_{t',t}^m(2) + \zeta_{t, \quant}^m(2)) \right\}\right]
\end{align}

In order to further simplify the above equation, we first need to analyze the term $(\E[x_{t, \max}^m] - \E[\xi_{t',t, \max}^m])$ using the relation in Eqn.~\eqref{eqn:delta_max_unaveraged_expectation_lower_bound}. To analyze that expression, we consider the following recursive relation for any fixed client $m$:
\begin{align}
    y_t = (1- \eta_t)y_{t-1} + \eta_t(\gamma  y_{t-1} + \E[\xi_{t',t, \max}^m]). \label{eqn:y_recursion}
\end{align}
Note that $\E[\xi_{t',t, \max}^m]$ is a constant which we will bound later. Upon unrolling the recursion, we obtain,
\begin{align}
    y_t = \left(\prod_{k = t' +1}^t (1- \eta_k) \right) y_{t'}  +  \sum_{k = t' + 1}^t \left( \eta_k  \prod_{i = k+1}^t (1- \eta_i) \right) \gamma  y_{k-1}  + \sum_{k = t' + 1}^t \left( \eta_k  \prod_{i = k+1}^t (1- \eta_i) \right) \E[\xi_{t',t, \max}^m].\label{eqn:y_recursion_unrolled}
\end{align}
On the other hand, Eqn.~\eqref{eqn:delta_max_unaveraged_expectation_lower_bound} can be written as
\begin{align*}
    \E[x_{t, \max}^m] & \geq \varphi_{t', t}  \E[\barx_{t', \max}] +  \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \E[\max\{|\bfx_{k-1}^m(1)|, |\bfx_{k-1}^m(2)|\}]  \right] + \E[\xi_{t',t, \max}^m] - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|] \\
    & \geq \varphi_{t', t}  \E[\barx_{t', \max}] +  \left[\sum_{k = t' + 1}^t  \lambda_{k, t}\gamma \E[x_{k-1, \max}^m]  \right] + \E[\xi_{t',t, \max}^m] - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|].
\end{align*}
Using the above expression, it is straightforward to note that if the recursion in Eqn.~\eqref{eqn:y_recursion} is initialized with $y_{t'} = \E[\barx_{t', \max}]$, then $\E[x_{t, \max}^m] \geq y_t - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|]$ as $\sum_{k = t' + 1}^t \left( \eta_k  \prod_{i = k+1}^t (1- \eta_i) \right) = \sum_{k = t' + 1}^t \widetilde{\eta}_k^{(t)}  \leq 1$ (See Eqn.~\eqref{eqn:tilde_eta_k_t_recursion}). By rewriting Eqn.~\eqref{eqn:y_recursion} as
\begin{align*}
    y_t = (1- \eta_t(1-\gamma ))y_{t-1} + \eta_t \E[\xi_{t',t, \max}^m],
\end{align*}
it is straight forward to note that $y_t$ is given as
\begin{align}
    y_t =  \left(\prod_{k = t' + 1}^t (1 - \eta_k(1-\gamma))\right) y_{t'} + \E[\xi_{t',t, \max}^m] \left[\sum_{k = t' + 1}^t  \eta_k^{(t)} \right]. \label{eqn:y_recursion_solved}
\end{align}
Consequently, we have,
\begin{align}
    \E[x_{t, \max}^m] - \E[\xi_{t',t, \max}^m] \geq  \left(\prod_{k = t' + 1}^t (1 - \eta_k(1-\gamma))\right) \E[\barx_{t', \max}] + \E[\xi_{t',t, \max}^m] \left[\sum_{k = t' + 1}^t \eta_k^{(t)} - 1  \right] - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|]. \label{eqn:delta_minus_xi_eqn_1}
\end{align}
We can slightly tighten the lower bound above as follows. Consider the recursive sequence defined as
\begin{align}
    w_t = (1- \eta_t)w_{t-1} + \eta_t(\gamma  w_{t-1}). \label{eqn:w_recursion}
\end{align}
Using a similar sequence of arguments as outlined in Eqns.~\eqref{eqn:y_recursion}-\eqref{eqn:y_recursion_solved}, we can conclude that
if $w_{t'} = \E[\barx_{t', \max}]$, then $\E[x_{t, \max}^m] \geq w_t + \E[\xi_{t',t, \max}^m] -  \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|]$ and consequently,
\begin{align}
    \E[x_{t, \max}^m] & \geq (1 - \eta_{\tau}(1-\gamma ))^{t - t'} \E[\barx_{t', \max}] + \E[\xi_{t',t, \max}^m] - \varphi_{t', t} \E[|\barDelta_{t'}(1) - \barDelta_{t'}(2)|]. \label{eqn:delta_minus_xi_eqn_2}
\end{align}
Thus, combining Eqns.~\eqref{eqn:delta_minus_xi_eqn_1} and~\eqref{eqn:delta_minus_xi_eqn_2} yields,
\begin{align}
    \E[x_{t, \max}^m] - \E[\xi_{t',t, \max}^m] \geq  \left(\prod_{k = t' + 1}^t (1 - \eta_k(1-\gamma))\right) \E[\barx_{t', \max}] + \E[\xi_{t',t, \max}^m] \left[\sum_{k = t' + 1}^t \eta_k^{(t)} - 1  \right]_{+} - \varphi_{t', t} \E[|\barbfx_{t'}(1) - \barbfx_{t'}(2)|], \label{eqn:delta_minus_xi}
\end{align}
where $[x]_{+} = \max\{x, 0\}$. The following lemmas provide bounds on the individual terms in the above expression.
\begin{lemma}
    For all consecutive averaging instants $t', t$ and all $m \in \{1,2,\dots, M\}$,
    \begin{align*}
        \E[\xi_{t',t, \max}^m] & \geq \frac{\sigma}{8} \sqrt{\frac{1}{B\ln 2} \sum_{k = t' + 1}^t \left(\widetilde{\eta}_{k}^{(t)} \right)^2}, \\
        \E\left[\max\left\{ \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(1), \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(2) \right\}\right] & \geq \frac{\sigma}{8} \sqrt{\frac{1}{BM\ln 2} \sum_{k = t' + 1}^t \left(\widetilde{\eta}_{k}^{(t)} \right)^2} .
    \end{align*}
    Furthermore, if $t - \max\{t' , \tau\} \geq 1/\eta_{\tau}$, then
    \begin{align*}
    \E[\xi_{t',t, \max}^m] & \geq \frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 B\ln 2} }, \\
    \E\left[\max\left\{ \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(1), \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(2) \right\}\right] & \geq
    \frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 BM\ln 2} }. 
\end{align*}
    \label{lemma:xi_lower_bound}
\end{lemma}


\begin{lemma}
    For all $t \in \{t_r\}_{r = 1}^R$, we have 
    \begin{align*}
         \E[|\barbfx_{t}(1) - \barbfx_{t}(2)|] \leq \sigma \sqrt{\frac{12\eta_T}{BM}}.
    \end{align*}
    \label{lemma:barDelta_action_diff}
\end{lemma}

\begin{lemma}
    For all $t, t' \geq \tau$ such that $t - t' \geq 8/\eta_{\tau}$,
    \begin{align*}
        \sum_{k = t' + 1}^t \eta_k^{(t)} - 1 \geq \frac{1 - (1-\eta_{\tau}(1-\gamma))^{t - t'}}{24(1-\gamma)}.
    \end{align*}
    \label{lemma:eta_k_t_sum_minus_1}
\end{lemma}

Thus, on combining the results from Lemmas~\ref{lemma:xi_lower_bound},~\ref{lemma:barDelta_action_diff},~\ref{lemma:eta_k_t_sum_minus_1} and Eqn.~\eqref{eqn:delta_minus_xi} and plugging them into Eqn.~\eqref{eqn:barDelta_max_as_func_clients}, we obtain the following relation for $t, t' \geq \tau$:
\begin{align}
    \E[\barx_{t, \max}] & \geq (1 - \eta_{\tau}(1-\gamma))^{t-t'}\E[\barx_{t', \max}] + \left( \frac{1 - (1-\eta_{\tau}(1-\gamma))^{t - t'}}{24(1-\gamma)}\right)\frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 B\ln 2} } \cdot \1\{t - t' \geq 8/\eta_{\tau}\} \nonumber\\
    & ~~~~~~~~~ - 2(1-\eta_T)^{t-t'} \sigma \sqrt{\frac{12\eta_T}{BM}}  + \frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 BM\ln 2} } \cdot \1\{t - t' \geq 8/\eta_{\tau}\} \label{eqn:barDelta_recursion}
\end{align}

We are interested in evaluating $\E[\barx_{T, \max}]$. To this effect, we introduce some notation to simplify the presentation. Let $R_{\tau} := \min \{r : t_r \geq \tau \}$. For the constant step size schedule, we have, $R_{\tau} = 0$, with $t_0 = 0$ (as all agents start at the same point). For the rescaled linear step size, we temporarily assume that $R_{\tau} \leq 2T/3$. We later consider the case where $R_{\tau} > 2T/3$. For $r = R_{\tau},\dots, R$, we define the following terms
\begin{align*}
    \zeta_r & := \E[\barx_{t_r, \max}] \\
    \alpha_r & := (1 - \eta_{\tau}(1-\gamma))^{t_r - t_{r-1}} \\
    \beta_r & := (1 - \eta_T)^{t_r - t_{r-1}} \\
    \cI_r & := \{r \geq r' > R_{\tau} : t_{r'} - t_{r'-1} \geq 8/\eta_{\tau}\} \\
    C_1 & :=  \frac{\sigma}{192(1-\gamma)} \sqrt{\frac{\eta_T}{5 B\ln 2} } \\
    C_2 & := \sigma \sqrt{\frac{48\eta_T}{BM}} \\
    C_3 & := \frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 BM\ln 2} }.
\end{align*}

We these notations in place, the recursion in Eqn.~\eqref{eqn:barDelta_recursion} can be rewritten as
\begin{align}
    \zeta_r \geq \alpha_r \zeta_{r-1} - \beta_r C_2 + C_3 \1 \{r \in \cI_r \} + (1 - \alpha_r) C_1 \1 \{r \in \cI_r \}, \label{eqn:zeta_recursion}
\end{align}
for all $r \geq R_{\tau}$. We claim that $\zeta_r$ satisfies the following relation for all $r \geq R_{\tau} + 1$.
\begin{align}
    \zeta_r \geq \left( \prod_{i = R_{\tau}+1}^r \alpha_i \right) \zeta_{R_{\tau}} - \sum_{k = R_{\tau}+1}^r  \beta_k \left( \prod_{i = k+1}^{r} \alpha_i \right) C_2 + \sum_{k = R_{\tau} +1 }^r   \left( \prod_{i = k+1}^{r} \alpha_i \right)  \1\{k \in \cI_k\} C_3 + C_1 \left( \prod_{i \notin \cI_r} \alpha_i \right) \left( 1 - \prod_{i \in \cI_r} \alpha_i \right), \label{eqn:zeta_recursion_solved}
\end{align}
where recall that if there is no valid index for a product, its value is taken to be $1$. We use induction to prove the claim is true. For the base case, Eqn.~\eqref{eqn:zeta_recursion} yields
\begin{align}
    \zeta_{R_{\tau}+1} & \geq \alpha_{R_{\tau}+1} \zeta_{R_{\tau}} - \beta_{R_{\tau}+1} C_2 + C_3 \1\{R_{\tau} + 1 \in \cI_{R_{\tau} + 1}\} + (1 - \alpha_{R_{\tau}+1}) C_1 \1 \{{R_{\tau}+1} \in \cI_{R_{\tau}+1} \}.
\end{align}
Note that this is identical to the expression in Eqn.~\eqref{eqn:zeta_recursion_solved} for $r = R_{\tau} +1$ as 
\begin{align*}
    \left( \prod_{i \notin \cI_{R_{\tau}+1}} \alpha_i \right) \left( 1 - \prod_{i \in \cI_{R_{\tau}+1}} \alpha_i \right) = (1 - \alpha_{R_{\tau}+1}) \1 \{{R_{\tau}+1} \in \cI_{R_{\tau}+1} \},
\end{align*}
based on the adopted convention for products with no valid indices. For the induction step, assume Eqn.~\eqref{eqn:zeta_recursion_solved} holds for $r$. On combining Eqns.~\eqref{eqn:zeta_recursion} and~\eqref{eqn:zeta_recursion_solved}, we obtain,
\begin{align}
    \zeta_{r+1} & \geq \alpha_{r+1} \zeta_{r} - \beta_{r+1} C_2 + C_3 \1 \{(r+1) \in \cI_{r+1} \}  + (1 - \alpha_{r+1}) C_1 \1 \{r+1 \in \cI_{r+1} \} \nonumber \\
    & \geq \alpha_{r+1} \left( \prod_{i = R_{\tau} + 1}^r \alpha_i \right) \zeta_{R_{\tau}} - \alpha_{r+1}  \sum_{k = R_{\tau} + 1}^r  \beta_k \left( \prod_{i = k+1}^{r} \alpha_i \right) C_2 + \alpha_{r+1} \sum_{k = R_{\tau} + 1}^r   \left( \prod_{i = k+1}^{r} \alpha_i \right) C_3 \1\{k \in \cI_k\}  \nonumber \\
    &  + \alpha_{r+1} C_1 \left( \prod_{i \notin \cI_r} \alpha_i \right) \left( 1 - \prod_{i \in \cI_r} \alpha_i \right) - \beta_{r+1} C_2 + C_3 \1 \{(r+1) \in \cI_{r+1} \} + (1 - \alpha_{r+1}) C_1 \1 \{(r+1) \in \cI_{r+1} \} \nonumber \\
    & \geq \left( \prod_{i = R_{\tau} + 1}^{r+1} \alpha_i \right) \zeta_{R_{\tau}} -  \sum_{k = R_{\tau} + 1}^{r+1}  \beta_k \left( \prod_{i = k+1}^{r+1} \alpha_i \right) C_2 + \sum_{k = R_{\tau} + 1}^{r+1}   \left( \prod_{i = k+1}^{r+1} \alpha_i \right) C_3 \1\{k \in \cI_k\} \nonumber \\
    & ~~~~~~~~~ + \alpha_{r+1} C_1 \left( \prod_{i \notin \cI_r} \alpha_i \right) \left( 1 - \prod_{i \in \cI_r} \alpha_i \right)  + (1 - \alpha_{r+1}) C_1 \1 \{(r+1) \in \cI_{r+1} \}. \label{eqn:zeta_induction_step}
\end{align}
If $(r+1) \notin \cI_{r+1}$, then $\left( 1 - \prod_{i \in \cI_r} \alpha_i \right) = \left( 1 - \prod_{i \in \cI_{r+1}} \alpha_i \right)$ and $\alpha_{r+1} \left( \prod_{i \notin \cI_r} \alpha_i \right) = \left( \prod_{i \notin \cI_{r+1}} \alpha_i \right)$. Consequently, 
\begin{align}
    \alpha_{r+1} C_1 \left( \prod_{i \notin \cI_r} \alpha_i \right) \left( 1 - \prod_{i \in \cI_r} \alpha_i \right)  + (1 - \alpha_{r+1}) C_1 \1 \{(r+1) \in \cI_{r+1} \} = C_1 \left( \prod_{i \notin \cI_{r+1}} \alpha_i \right) \left( 1 - \prod_{i \in \cI_{r+1}} \alpha_i \right). \label{eqn:r_plus_one_not_in_I}
\end{align}
On the other hand, if $(r+1) \in \cI_{r+1}$, then $\left( \prod_{i \notin \cI_r} \alpha_i \right) = \left( \prod_{i \notin \cI_{r+1}} \alpha_i \right)$. Consequently, we have,
\begin{align}
    &\alpha_{r+1} C_1 \left( \prod_{i \notin \cI_r} \alpha_i \right) \left( 1 - \prod_{i \in \cI_r} \alpha_i \right)  + (1 - \alpha_{r+1}) C_1 \1 \{(r+1) \in \cI_{r+1} \} \nonumber \\
    &  = \alpha_{r+1} C_1 \left( \prod_{i \notin \cI_{r+1}} \alpha_i \right) \left( 1 - \prod_{i \in \cI_r} \alpha_i \right)  + (1 - \alpha_{r+1}) C_1 \nonumber \\
    &  \geq  C_1 \left( \prod_{i \notin \cI_{r+1}} \alpha_i \right) \left[\alpha_{r+1}\left( 1 - \prod_{i \in \cI_r} \alpha_i \right)  + (1 - \alpha_{r+1}) \right] \nonumber \\
    &  \geq  C_1 \left( \prod_{i \notin \cI_{r+1}} \alpha_i \right) \left( 1 - \prod_{i \in \cI_{r+1}} \alpha_i \right). \label{eqn:r_plus_one_in_I}
\end{align}
Combining Eqns.~\eqref{eqn:zeta_induction_step},~\eqref{eqn:r_plus_one_not_in_I} and~\eqref{eqn:r_plus_one_in_I} proves the claim. \\

Invoking Eqn.~\eqref{eqn:zeta_recursion_solved} for $r = R$ and using the relation $\zeta_{R_{\tau}} \geq 0$, we obtain,
\begin{align}
    \zeta_R & \geq - \sum_{k = R_{\tau}+1}^{R}  \beta_k \left( \prod_{i = k+1}^{R} \alpha_i \right) C_2 + \sum_{k = R_{\tau} +1 }^R   \left( \prod_{i = k+1}^{R} \alpha_i \right) C_3 \1\{k \in \cI_k\} + C_1 \left( \prod_{i \notin \cI_R} \alpha_i \right) \left( 1 - \prod_{i \in \cI_R} \alpha_i \right), \nonumber \\
    & \geq - R C_2  + C_1 \left( \prod_{i \notin \cI_R} \alpha_i \right) \left( 1 - \prod_{i \in \cI_R} \alpha_i \right) \nonumber \\
    & \geq - R \cdot \sigma\sqrt{\frac{48\eta_T}{BM}}  +  \left( \prod_{i \notin \cI_R} \alpha_i \right) \left( 1 - \prod_{i \in \cI_R} \alpha_i \right) \cdot \frac{\sigma}{192} \sqrt{\frac{\eta_T}{5 B\ln 2} }, \label{eqn:zeta_R_final}
\end{align}
where we used the fact $\beta_k \left( \prod_{i = k+1}^{R} \alpha_i \right) \leq 1$ and that $C_3 \geq 0$. Consider the expression
\begin{align}
    \prod_{i \notin \cI_R} \alpha_i & = \prod_{i \notin \cI_R} (1 - \eta_{\tau}(1- \gamma))^{t_{i} - t_{i-1}} \geq 1 - \eta_{\tau}(1- \gamma) \cdot \underbrace{\sum_{i \notin \cI_R} (t_{i} - t_{i-1})}_{ := T_1} . \label{eqn:alpha_i_prod}
\end{align}
Consequently, 
\begin{align}
    \left( 1 - \prod_{i \in \cI_R} \alpha_i \right) = 1 - (1 - \eta_{\tau}(1- \gamma ))^{T - t_{R_{\tau}} - T_1} \geq 1 - \exp \left( - \eta_{\tau} (1- \gamma ) \left(T - t_{R_{\tau}} - T_1 \right)\right) \label{eqn:one_minus_alpha_i_prod}
\end{align}
Note that $T_1$ satisfies the following bound
\begin{align}
    T_1 : = \sum_{i \notin \cI_R} (t_{i} - t_{i-1}) \leq (R - |\cI_R|) \cdot \frac{8}{\eta_{\tau}} \leq \frac{8R}{\eta_{\tau}}. \label{eqn:T_1_bound}
\end{align}

We split the remainder of the analysis based on the step size schedule. We begin with considering the case with constant step size i.e, $\eta_t = \eta \geq \frac{1}{(1-\gamma)T}$. for all $t$. Under this scenario, we have $\tau = 0$. If $R \leq \frac{1}{8000(1-\gamma)}$ then, Eqns.~\eqref{eqn:alpha_i_prod},~\eqref{eqn:one_minus_alpha_i_prod} and~\eqref{eqn:T_1_bound} yield the following relations:
\begin{align*}
    T_1 & \leq \frac{8R}{\eta} \leq \frac{T}{1000}, \\
    \prod_{i \notin \cI_R} \alpha_i & \geq 1 - \eta (1- \gamma ) \cdot T_1 \geq 1 - 8R(1 -\gamma) \geq 0.999 \\
    \left( 1 - \prod_{i \in \cI_R} \alpha_i \right) & \geq 1 - \exp \left( - \eta (1- \gamma ) \left(T  - T_1 \right)\right) \geq 1 - \exp \left( - 0.999\right).
\end{align*}
On plugging the above relations into Eqn.~\eqref{eqn:zeta_R_final}, for any $M \geq 2$ we obtain
\begin{align}
    \zeta_R & \geq \frac{\sigma}{1000(1-\gamma)} \sqrt{\frac{\eta_T}{B}} \nonumber \\
    & \geq \frac{\sigma}{1000} \sqrt{\frac{1}{(1-\gamma)^3BT}}. \label{eqn:zeta_R_bound_constant}
\end{align}

Similarly, we consider the rescaled linear step size schedule. As mentioned earlier, we take $\tau = T/3$ and $t_{R_{\tau}} \leq 2T/3$ for this case. Also, we take $c_{\eta}(1-\gamma)T \geq 1$ otherwise the analysis is almost identical to that for the constant step size. If $R \leq \frac{1}{8000(1-\gamma)  \max\{1,c_{\eta}\}}$ then, Eqns.~\eqref{eqn:alpha_i_prod},~\eqref{eqn:one_minus_alpha_i_prod} and~\eqref{eqn:T_1_bound} yield the following relations:
\begin{align*}
    T_1 & \leq \frac{8R}{\eta_{\tau}} \leq \frac{8R}{\eta_{T}} \leq \frac{T}{4000} \\
    \prod_{i \notin \cI_R} \alpha_i & \geq 1 - \eta_{\tau} (1- \gamma p) \cdot T_1 \geq 1 - 8R(1 -\gamma) \geq 0.999 \\
    \left( 1 - \prod_{i \in \cI_R} \alpha_i \right) & \geq 1 - \exp \left( - \eta_{T} (1- \gamma ) \left(\frac{T}{3}  - T_1 \right)\right) \geq 1 - \exp \left( -  \frac{3}{4}\left(\frac{1}{3}  - \frac{1}{4000} \right)\right).
\end{align*}
On plugging the above relations into Eqn.~\eqref{eqn:zeta_R_final}, we obtain
\begin{align}
    \zeta_R &  \geq \frac{3\sigma}{5000(1-\gamma)\max\{1,c_{\eta}\}} \sqrt{\frac{\eta_T}{B}} \nonumber \\ 
    & \geq \frac{3\sigma}{5000(1-\gamma)\max\{1,c_{\eta}\}} \sqrt{\frac{1}{(1-\gamma)BT}}.  \label{eqn:zeta_R_bound_linear}
\end{align}

Let us consider the case when $t_{R_{\tau}} > 2T/3$. The condition $t_{R_{\tau}} > 2T/3$ implies that the time between the communication rounds $R_{\tau} - 1$ and $R_{\tau}$ is at least $T/3$. Thus, Eqn.~\eqref{eqn:barDelta_recursion} yields that
\begin{align}
    \E[\barx_{t_{R_{\tau}}}] \geq \left( \frac{1 - (1-\eta_{\tau}(1-\gamma))^{T/3}}{24(1-\gamma)}\right)\frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 B\ln 2} }  - 2(1-\eta_T)^{T/3} \sigma \sqrt{\frac{12\eta_T}{BM}}.
\end{align}
On plugging in the values of $\eta_{\tau}$ and $\eta_T$ and using similar steps as used in the previous case, we can conclude that for all $M \geq 2$
\begin{align}
    \E[\barx_{t_{R_{\tau}}}] \geq c_1 \frac{\sigma}{1-\gamma}\sqrt{\frac{\eta_T}{B}}
\end{align}
holds for some universal constant $c_1 \geq 0$. Even if all th

Thus, Eqns.~\eqref{eqn:zeta_R_bound_constant} and~\eqref{eqn:zeta_R_bound_linear} together imply that there exists a numerical constant $c_0 > 0$ such that 
\begin{align}
    \ER(\sA; N, M) = \E[\|\bfx_T^m - \bfx_{\star}\|_{\infty}] \geq \E[\barx_{T, \max}] \geq c_0 \sigma \sqrt{\frac{1}{(1-\gamma)^3N}}. \label{eqn:err_large_lr_final_bound}
\end{align}








\subsubsection{Proof of Lemma~\ref{lemma:xi_lower_bound}}

Using the relation $\max\{a,b\} = \dfrac{a + b + |a - b|}{2}$, we can rewrite $\E[\xi_{t',t,\max}^m]$ as 
\begin{align*}
    \E[\xi_{t',t, \max}^m] & = \E\left[ \frac{\xi_{t',t}^m(1) + \xi_{t',t}^m(2)}{2} + \left| \frac{\xi_{t',t}^m(1) - \xi_{t',t}^m(2)}{2} \right| \right] \\
    & = \frac{1}{2} \E\left[\left| \frac{\xi_{t',t}^m(1) - \xi_{t',t}^m(2)}{2} \right| \right] \\
    & = \frac{1}{2} \E\left[\left| \sum_{k = t' + 1}^t \widetilde{\eta}_{k}^{(t)} (\hatbfz_k^m(1) - \hatbfz_k^m(2)) \right| \right],
\end{align*}
where we used the fact that $\E[\xi_{t',t}^m(1)] = \E[\xi_{t',t}^m(2)] = 0$. From the definition of $\bfz$, we have $\text{Var}(\bfz(i)) = \sigma^2$ and $\bfz(i)$ is $\sigma^2$-sub-Gaussian for $i = 1, 2$. Consequently, $\text{Var}(\hatbfz(i)) = \frac{\sigma^2}{B}$ and $\hatbfz(i)$ is $\frac{\sigma^2}{B}$-sub-Gaussian for $i = 1, 2$. Furthermore, using the independence of noise variables across clients and time instances, we can conclude that $\sum_{k = t' + 1}^t \widetilde{\eta}_{k}^{(t)} (\hatbfz_k^m(1) - \hatbfz_k^m(2))$ is also sub-Gaussian random variable with variance and variance proxy both equal to $\frac{2\sigma^2}{B} \sum_{k = t' + 1}^t \left(\widetilde{\eta}_{k}^{(t)} \right)^2$.  \\

The following lemma, whose proof is deferred to Sec.~\ref{proof:sub_gaussian_lower_bound}, provides a lower bound on the absolute value of a sub-Gaussian random variable.

\begin{lemma}
    Let $X$ be a zero mean random variable satisfying $\E[X^2] = \sigma_{\text{var}}^2$ and $\E[\exp(\lambda X)] \leq \exp(\lambda^2 \sigma_{\text{subG}}^2/2)$ for all $\lambda \in \R$, i.e., $X$ is $\sigma_{\text{subG}}^2$-sub-Gaussian. Then, 
    \begin{align*}
        \E[|X|] & \geq \frac{\sigma_{\text{var}}^2}{2 \sigma_{\text{subG}}} \cdot \frac{1}{\sqrt{2 \ln \left( \frac{8\sigma_{\text{subG}}^2}{\sigma_{\text{var}}^2}\right)}}
    \end{align*}
    \label{lemma:sub_gaussian_lower_bound}
\end{lemma}

Thus, using the result from Lemma~\ref{lemma:sub_gaussian_lower_bound}, along with the values of variance and variance proxy, we can conclude that
\begin{align}
    \E[\xi_{t',t, \max}^m] \geq \frac{\sigma}{8} \sqrt{\frac{1}{B\ln 2} \sum_{k = t' + 1}^t \left(\widetilde{\eta}_{k}^{(t)} \right)^2 }.
    \label{eqn:xi_expected_value_expression}
\end{align}

Using an identical argument, we can conclude that,
\begin{align}
    \E\left[\max\left\{ \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(1), \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(2) \right\}\right] & \geq \frac{\sigma}{8} \sqrt{\frac{1}{BM\ln 2} \sum_{k = t' + 1}^t \left(\widetilde{\eta}_{k}^{(t)} \right)^2}. \label{eqn:xi_expected_value_expression_client averaged}
\end{align}

For $t - \max\{t', \tau\} \geq 1/\eta_{\tau}$, we have,
\begin{align}
    \sum_{k = t' + 1}^t \left(\widetilde{\eta}_{k}^{(t)}\right)^2 & \geq \sum_{k = \max\{t', \tau\} + 1}^t \left(\widetilde{\eta}_{k}^{(t)}\right)^2 \nonumber \\
    & \geq \sum_{k = \max\{t', \tau\} + 1}^t \left( \eta_k \prod_{i = k+1}^t (1- \eta_i) \right)^2 \nonumber  \\
    & \geq \sum_{k = \max\{t', \tau\} + 1}^t \left( \eta_t \prod_{i = k+1}^t (1- \eta_{\tau}) \right)^2 \nonumber  \\
    & \geq \eta_t^2 \sum_{k = \max\{t', \tau\} + 1}^t (1- \eta_{\tau})^{2(t-k)} \nonumber  \\
    & \geq \eta_t^2 \cdot \frac{1 - (1-\eta_{\tau})^{2(t-\max\{t', \tau\})}}{\eta_{\tau}(2 - \eta_{\tau})} \nonumber  \\
    & \geq \eta_t \cdot \frac{1 - \exp(-2)}{4} \nonumber   \\
    & \geq \frac{\eta_t}{5} \geq \frac{\eta_T}{5}.
    \label{eqn:lambda_square_sum_lower_bound}
\end{align}
On plugging the above result in Eqns.~\eqref{eqn:xi_expected_value_expression} and~\eqref{eqn:xi_expected_value_expression_client averaged}, we obtain,
\begin{align*}
    \E[\xi_{t',t, \max}^m] & \geq \frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 B\ln 2} }, \\
    \E\left[\max\left\{ \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(1), \frac{1}{M}\sum_{m = 1}^M \xi_{t',t}^m(2) \right\}\right] & \geq
    \frac{\sigma}{8} \sqrt{\frac{\eta_T}{5 BM\ln 2} }. 
\end{align*}


\subsubsection{Proof of Lemma~\ref{lemma:barDelta_action_diff}}

Using Eqns.~\eqref{eqn:delta_m_averaged} and~\eqref{eqn:xi_def}, we can write
\begin{align*}
    \barbfx_t(1) - \barbfx_t(2) = \left(\prod_{k = t' +1}^t (1- \eta_k)\right) (\barbfx_{t'}(1) - \barbfx_{t'}(2)) + \frac{1}{M} \sum_{m = 1}^M \sum_{k = t' + 1}^t \widetilde{\eta}_{k}^{(t)} (\hatbfz_k^m(1) - \hatbfz_k^m(2)) %+ \frac{1}{M} \sum_{m = 1}^M (\zeta_{t, \quant}^m(1) - \zeta_{t, \quant}^m(2)).
\end{align*}
Upon unrolling the recursion, we obtain,
\begin{align*}
    \barbfx_t(1) - \barbfx_t(2) =  \frac{1}{M} \sum_{k = 1}^t \sum_{m = 1}^M  \widetilde{\eta}_{k}^{(t)} (\hatbfz_k^m(1) - \hatbfz_k^m(2)) %+ \frac{1}{M} \sum_{r = 1}^R \sum_{m = 1}^M \left(\prod_{k = t_r +1}^{t} (1- \eta_k)\right) (\zeta_{t_r, \quant}^m(1) - \zeta_{t_r, \quant}^m(2)).
\end{align*}
If we define a filtration $\sF_k$ as the $\sigma$-algebra corresponding to $\{\hatbfz_l^1(1), \hatbfz_l^1(2), \dots, \hatbfz_l^M(1), \hatbfz_l^M(2)\}_{l = 1}^k$, then it is straightforward to note that $\{\barbfx_t(1) - \barbfx_t(2)\}_{t}$ is a martingale sequence adapted to the filtration $\{\sF_t\}_{t}$. Consequently, $\{|\barbfx_t(1) - \barbfx_t(2)|\}_{t}$ is a sub-martingale adapted to  the same filtration. As a result, 
\begin{align}
    \sup_{1 \leq t \leq T} \E[|\barbfx_t(1) - \barbfx_t(2)|] & \leq \E[|\barbfx_T(1) - \barbfx_T(2)|]  \leq \left(\E[(\barbfx_T(1) - \barbfx_T(2))^2] \right)^{1/2}. \label{eqn:sub_martingale} 
\end{align}
Once again, on using the independence of noise variables across clients and time instances, we can conclude that
\begin{align}
    \E[(\barbfx_T(1) - \barbfx_T(2))^2] & = \E\left[ \left( \frac{1}{M} \sum_{k = 1}^T \sum_{m = 1}^M  \widetilde{\eta}_{k}^{(t)} (\hatbfz_k^m(1) - \hatbfz_k^m(2)) \right)^2 \right] \nonumber \\
    & = \frac{1}{M^2} \E\left[  \sum_{k = 1}^T \sum_{m = 1}^M  \left(\widetilde{\eta}_{k}^{(t)}\right)^2 \E(\hatbfz_k^m(1))^2] + \E[(\hatbfz_k^m(2))^2] \right] \nonumber \\
    & = \frac{\sigma^2}{BM} \E\left[  \sum_{k = 1}^T \left( \eta_k \prod_{i = k+1}^T (1- \eta_i) \right)^2  \right]. \label{eqn:martingale_sum_of_squares}
\end{align}
Let us focus on the term involving the step sizes. We have,
\begin{align}
    \sum_{k = 1}^T   \left( \eta_k \prod_{i = k+1}^T (1- \eta_i) \right)^2 & = \sum_{k = 1}^{\tau}   \left( \eta_k \prod_{i = k+1}^T (1- \eta_i) \right)^2 + \sum_{k = \tau+1}^{T}   \left( \eta_k \prod_{i = k+1}^T (1- \eta_i) \right)^2 \nonumber \\
    & \leq \sum_{k = 1}^{\tau}  (1- \eta_{\tau})^{2(T-k)} + \sum_{k = \tau+1}^{T}    \eta_k^2 (1- \eta_T)^{2(T-k)}  \nonumber \\
    & \leq  \frac{(1- \eta_{\tau})^{2(T-\tau)}(1 - (1- \eta_{\tau})^{2\tau})}{\eta_{\tau}} + \eta_{\tau}^2 \cdot  \frac{(1 - (1- \eta_{T})^{2(T-\tau)})}{\eta_{T}}  \nonumber \\
    & \leq  \eta_{\tau} + 3\eta_{\tau}   \nonumber \\
    & \leq  12\eta_{T}, \label{eqn:eta_squares_sum}
\end{align}
where the first term in the fourth step follows from the condition on $T$ and the bound $\eta_{\tau} \geq \frac{1}{(1-\gamma)T}$. On combining Eqns.~\eqref{eqn:sub_martingale},~\eqref{eqn:martingale_sum_of_squares} and~\eqref{eqn:eta_squares_sum}, we obtain
\begin{align*}
    \sup_{1 \leq t \leq T} \E[|\barbfx_t(1) - \barbfx_t(2)|] & \leq \sigma \sqrt{\frac{12\eta_T}{BM}},
\end{align*}
as required.





\subsubsection{Proof of Lemma~\ref{lemma:sub_gaussian_lower_bound}}
\label{proof:sub_gaussian_lower_bound}

For any $K > 0$, we have,
\begin{align*}
    \E[|X|] & \geq \E[|X|\1\{|X| \leq K\}] \\
    & \leq \frac{1}{K} \E[|X|^2\1\{|X| \leq K\}] \\
    & \leq \frac{1}{K} \left( \E[|X|^2] - \E[|X|^2\1\{|X| > K\}] \right) \\
    & \leq \frac{1}{K} \left( \sigma_{\text{var}}^2 - \E[|X|^2\1\{|X| > K\}] \right).
\end{align*}
Thus, in order to lower bound the above expression, we need to find an upper bound for $\E[|X|^2\1\{|X| > K\}]$. We have,
\begin{align*}
    \E[|X|^2\1\{|X| > K\}] & = \int_{0}^{\infty} \Pr(|X|^2\1\{|X| > K\} > t) \ \mathrm{d}t \\
    & = \int_{K^2}^{\infty} \Pr(|X|^2 > t) \ \mathrm{d}t \\
    & = \int_{K^2}^{\infty} \Pr(|X| > \sqrt{t}) \ \mathrm{d}t \\
    & \leq 2 \int_{K^2}^{\infty} \exp\left( -\frac{t}{2\sigma_{\text{subG}}^2} \right)  \ \mathrm{d}t \\
    & \leq 4 \sigma_{\text{subG}}^2  \exp\left( -\frac{K^2}{2\sigma_{\text{subG}}^2} \right).
\end{align*}
Thus, if we choose $\displaystyle K := \sigma_{\text{subG}} \sqrt{2 \ln \left( \frac{8\sigma_{\text{subG}}^2}{\sigma_{\text{var}}^2} \right)}$, then $\E[|X|^2\1\{|X| > K\}] \leq \dfrac{\sigma_{\text{var}}^2}{2}$. Consequently, 
\begin{align*}
    \E[|X|] \geq \frac{\sigma_{\text{var}}^2}{2 \sigma_{\text{subG}}} \cdot \frac{1}{\sqrt{2 \ln \left( \frac{8\sigma_{\text{subG}}^2}{\sigma_{\text{var}}^2}\right)}}.
\end{align*}


\section{Analysis of \DVR}

In this section, we prove Theorem~\ref{thm:fed_dvr_performance} that outlines the performance guarantees of the proposed \DVR algorithm. There are two main parts of the proof. The first part of the proof deals with establishing that for the given choice of parameters described in Sec.~\ref{ssub:parameter_setting}, the output of the algorithm is $\varepsilon$-optimal estimate of $\starQ$ with probability $1 - \delta$. The second part of proof deals with deriving the bounds on sample and communication complexity based on the choice of prescribed parameters. We begin with the second part, which is easier of the two.

\subsection{Establishing the sample and communication complexity bounds}

We begin with bounding $\CC_{\textsf{round}}$. From the description of \DVR, it is straightforward to note that each epoch, i.e., each call to the \RE routine, involves $L + 1$ rounds of communication, one for estimating $\cT\barQ$ and the remaining $L$ during the iterative updates of the Q-function. Since there are a total of $K$ epochs,
\begin{align*}
    \CC_{\textsf{round}}(\DVR; \varepsilon, M, \delta) \leq (L+ 1)K \leq \frac{16}{\eta(1-\gamma)} \log_2\left(\frac{1}{(1-\gamma)\varepsilon}\right),
\end{align*}
where the second bound follows from the prescribed choice of parameters. Similarly, since the quantization step is designed to compress each coordinate into $J$ bits, each message transmitted by an agents has a size of no more than $J \cdot |\cS| |\cA|$. Consequently,
\begin{align*}
    \CC_{\textsf{bit}}(\DVR; \varepsilon, M, \delta) & \leq J \cdot |\cS| |\cA| \cdot \CC_{\textsf{round}}(\DVR; \varepsilon, M, \delta) \\
    & \leq \frac{32|\cS|\cA|}{\eta(1-\gamma)} \log_2\left(\frac{1}{(1-\gamma)\varepsilon}\right) \log_2\left(\frac{70}{\eta(1-\gamma)}\sqrt{\frac{2}{M} \log\left(\frac{8KL|\cS||\cA|}{\delta} \right)}\right),
\end{align*}
where once again in the second step we plugged the value of $J$ from Sec.~\ref{ssub:parameter_setting}. \\

In order to establish the bound on sample complexity, note that during epoch $k$, each agent takes a total of $\lceil N_k/M\rceil + L \cdot B $ samples, where the first term corresponds to approximating $\tildeT_N(\barQ)$ and the second corresponds to the samples taken during the iterative update scheme. Thus, the total sample complexity is obtained by summing up over all the $K$ epochs. We have,
\begin{align*}
    \SC(\DVR; \varepsilon, M, \delta) & \leq \sum_{k = 1}^K  \left(\left\lceil \frac{N_k}{M}\right\rceil + L \cdot B\right) \\
    & \leq L\cdot B \cdot K + \frac{1}{M}\sum_{k = 1}^K N_k + M \\
    & \leq \frac{4608}{\eta M(1-\gamma)^3}\log_2\left(\frac{1}{(1-\gamma)\varepsilon}\right)\log\left(\frac{8KL|\cS||\cA|}{\delta} \right) + M \\
    & ~~~~~~~~~~~~ + \frac{19600}{M(1-\gamma)^2} \log\left(\frac{8KL|\cS||\cA|}{\delta} \right) \left( \sum_{k = 1}^{K_0} 4^k + \sum_{k = K_0 + 1}^K 4^{k- K_0} \right)\\
    & \leq \frac{4608}{\eta M(1-\gamma)^3}\log_2\left(\frac{1}{(1-\gamma)\varepsilon}\right)\log\left(\frac{8KL|\cS||\cA|}{\delta} \right) + M \\
    & ~~~~~~~~~~~~ + \frac{19600}{3M(1-\gamma)^2} \log\left(\frac{8KL|\cS||\cA|}{\delta} \right) \left( 4^{K_0} +  4^{K - K_0} \right)\\
    & \leq \frac{4608}{\eta M(1-\gamma)^3}\log_2\left(\frac{1}{(1-\gamma)\varepsilon}\right)\log\left(\frac{8KL|\cS||\cA|}{\delta} \right) + M \\
    & ~~~~~~~~~~~~ + \frac{78400}{3M(1-\gamma)^2} \log\left(\frac{8KL|\cS||\cA|}{\delta} \right) \left( \frac{1}{1-\gamma} +  \frac{1}{(1-\gamma)\varepsilon^2} \right)\\
    & \leq \frac{313600}{\eta M(1-\gamma)^3\varepsilon^2}\log_2\left(\frac{1}{(1-\gamma)\varepsilon}\right)\log\left(\frac{8KL|\cS||\cA|}{\delta} \right) + M.
\end{align*}

\subsection{Establishing the error guarantees}

In this section, we show that the Q-function returned by the \DVR algorithm is $\varepsilon$-optimal with probability at least $1-\delta$. We claim that the estimates of the Q-function generated by the algorithm across difference epochs satisfy the following relation for all $k \leq K$ with probability $1 - \delta$:
\begin{align}
    \|Q^{(k)} - \starQ\|_{\infty} \leq  \dfrac{2^{-k}}{1-\gamma}.
    \label{eqn:q_k_relation}
\end{align}
The required bound on $\|Q^{(K)} - \starQ\|_{\infty}$ immediately follows by plugging in the value of $K$. Thus, for the remainder of the section, we focus on establishing the above claim. \\

Firstly, note that the update scheme of variance reduced learning carried out during the \RE routine resembles that of the classic Q-learning scheme, i.e., fixed-point iteration, with a different operator defined as follows:
\begin{align}
    \cH(Q) := \cT(Q) - \cT(\barQ) + \tildeT_N(\barQ). \label{eqn:operator_h_definition}
\end{align}
Thus, The update scheme at step $l \geq 1$ in Eqn.~\eqref{eqn:q_l_update_rule} can then be written as
\begin{align}
    Q_l^{(m)} = (1-\eta) Q_{l-1} + \eta \widehat{\cH}_l^{(m)}(Q_{l-1}), \label{eqn:q_l_update_rule_with_h}
\end{align}
where $\widehat{\cH}_l^{(m)}(Q) := \hatT_l^{(m)}(Q) - \hatT_l^{(m)}(\barQ) + \tildeT_N(\barQ)$ is a stochastic, unbiased estimate of the operator $\cH$, similar to $\hatT_l^{(m)}(Q)$. Let $Q_{\cH}^{\star}$ denote the fixed point of $\cH$. Then the update scheme in Eqn.~\eqref{}, drives the sequence $\{Q_{l}\}_{l}$ to $Q_{\cH}^{\star}$. As long as $\|Q^{\star} - Q_{\cH}^{\star}\|_{\infty}$ is small, the required error $\|Q_l - Q^{\star}\|_{\infty}$ can also be controlled. The following lemmas formalize these ideas and pave the path to establish the claim in Eqn.~\eqref{eqn:q_k_relation}.

\begin{lemma}
    Consider the \normalfont{\RE} routine described in Alg.~\ref{alg:refine_estimate} and let $Q_{\cH}^{\star}$ denote the fixed point of the operator $\cH$ defined in Eqn.~\eqref{eqn:operator_h_definition}. Then the iterate generated by \RE at the end of $L$ variance reduced updates, i.e., $Q_L$, satisfies,
    \begin{align*}
        \|Q_L - \starQH\|_{\infty} \leq \frac{1}{6} \left(\| \barQ - \starQ\|_{\infty} + \| \starQ - \starQH\|_{\infty} \right) + \frac{D}{70}
    \end{align*}
    with probability $1- \frac{\delta}{2K}$.
    \label{lemma:q_l_star_q_h_err}
\end{lemma}

\begin{lemma}
    Consider the \normalfont{\RE} routine described in Alg.~\ref{alg:refine_estimate} and let $Q_{\cH}^{\star}$ denote the fixed point of the operator $\cH$ defined in Eqn.~\eqref{eqn:operator_h_definition}. The following relation holds with probability $1- \frac{\delta}{2K}$:
    \begin{align*}
        \|\starQH - \starQ\|_{\infty} \leq \| \barQ - \starQ\|_{\infty} \cdot \sqrt{\frac{8\kappa'}{N(1-\gamma)^2} } +  \sqrt{\frac{32\kappa'}{N(1-\gamma)^3}} + \frac{2\kappa'}{3N(1- \gamma)^2} + \frac{D}{70},
    \end{align*}
    where $\kappa' = \log\left(\frac{12K|\cS||\cA|}{\delta} \right)$.
    \label{lemma:star_q_h_star_q_err}
\end{lemma}

We defer the proofs of these Lemmas to Sec.~\ref{}. Using the results from Lemmas~\ref{lemma:q_l_star_q_h_err} and~\ref{lemma:star_q_h_star_q_err}, we obtain
\begin{align}
    \|Q^{(k)} - \starQ\|_{\infty} & \leq \|Q^{(k)} - \starQ_{\cH_k}\|_{\infty} + \|\starQH - \starQ_{\cH_k}\|_{\infty} \nonumber \\
    & \leq \frac{1}{6} \left(\| Q^{(k-1)} - \starQ\|_{\infty} + \| \starQ - \starQ_{\cH_k}\|_{\infty} \right) + \frac{D_k}{70} + \|\starQ_{\cH_k} - \starQ\|_{\infty} \nonumber \\
    & \leq \frac{1}{6} \left(\| Q^{(k-1)} - \starQ\|_{\infty} + 7\| \starQ - \starQ_{\cH_k}\|_{\infty} \right) + \frac{D_k}{70} \nonumber \\
    & \leq \| Q^{(k-1)} - \starQ\|_{\infty}  \left( \frac{1}{6} + \frac{7}{6}\sqrt{\frac{8\kappa'}{N_k(1-\gamma)^2} } \right) + \frac{7}{6}\left(\sqrt{\frac{32\kappa'}{N_k(1-\gamma)^3}} + \frac{2\kappa'}{3N_k(1- \gamma)^2}\right)+ \frac{13D_k}{420} \nonumber  \\
    & \leq \| Q^{(k-1)} - \starQ\|_{\infty}  \left( \frac{1}{6} + \frac{7}{6}\sqrt{\frac{8\kappa'}{N_k(1-\gamma)^2} } \right) + \frac{7}{6} \sqrt{\frac{50\kappa'}{N_k(1-\gamma)^3}}+ \frac{13D_k}{420}, \label{eqn:q_k_err_recursive_relation}
\end{align}
holds with probability $1- \frac{\delta}{K}$. We invoke Lemma~\ref{lemma:q_l_star_q_h_err} in the second step and Lemma~\ref{lemma:star_q_h_star_q_err} in the fourth step corresponding to the \normalfont{\RE} routine during the $k^{\text{th}}$ epoch. In the fifth step, we used the fact that $\frac{N_k(1-\gamma)^2}{\kappa'} \geq 1$. We use induction along with the recursive relation in Eqn.~\eqref{eqn:q_k_err_recursive_relation} to establish the required claim. Let us first consider the case $0 \leq k \leq K_0$. The base case, $\|Q^{(0)} - \starQ\|_{\infty} \leq \frac{1}{1-\gamma}$, holds by definition. Let us assume the relation holds for $k - 1$. Then, from Eqn.~\eqref{eqn:q_k_err_recursive_relation}, we have
\begin{align}
    \|Q^{(k)} - \starQ\|_{\infty} & \leq \| Q^{(k-1)} - \starQ\|_{\infty}  \left( \frac{1}{6} + \frac{7}{6}\sqrt{\frac{8\kappa'}{N_k(1-\gamma)^2} } \right) + \frac{7}{6} \sqrt{\frac{50\kappa'}{N_k(1-\gamma)^3}}+ \frac{13D_k}{420} \nonumber \\
    & \leq \frac{2^{-(k-1)}}{1-\gamma}  \left( \frac{1}{6} + 2^{-k} \cdot \frac{7}{6}\sqrt{\frac{8}{N_0} } \right) + 2^{-k} \cdot \frac{7}{6} \sqrt{\frac{50}{N_0(1-\gamma)}}+ \frac{104}{420} \cdot \frac{2^{-(k-1)}}{1-\gamma} \nonumber \\
    & \leq \frac{2^{-(k-1)}}{1-\gamma}  \left( \frac{1}{6} + \cdot \frac{7}{6}\sqrt{\frac{91}{2N_0} } + \frac{1}{4} \right) \nonumber \\
    & \leq \frac{2^{-k}}{1-\gamma}. \label{eqn:q_k_induction_case_1}
\end{align}
Now we move to the second case, for $k > K_0$.
% From Eqn.~\eqref{eqn:q_k_induction_case_1}, we know $\|Q^{(K_0)} - \starQ\|_{\infty} \leq \frac{1}{\sqrt{1-\gamma}}$, which establishes our base case. Consider any $k \geq K_0 + 1$. 
From Eqn.~\eqref{eqn:q_k_err_recursive_relation}, we have
\begin{align}
    \|Q^{(k)} - \starQ\|_{\infty} & \leq \| Q^{(k-1)} - \starQ\|_{\infty}  \left( \frac{1}{6} + \frac{7}{6}\sqrt{\frac{8\kappa'}{N_k(1-\gamma)^2} } \right) + \frac{7}{6} \sqrt{\frac{50\kappa'}{N_k(1-\gamma)^3}}+ \frac{13D_k}{420} \nonumber \\
    & \leq \frac{2^{-(k-1)}}{1-\gamma}  \left( \frac{1}{6} + 2^{-(k-K_0)} \cdot \frac{7}{6}\sqrt{\frac{8}{N_0} } \right) + 2^{-(k-K_0)} \cdot \frac{7}{6} \sqrt{\frac{50}{N_0(1-\gamma)}}+ \frac{104}{420} \cdot \frac{2^{-(k-1)}}{1-\gamma} \nonumber \\
    & \leq \frac{2^{-(k-1)}}{1-\gamma}  \left( \frac{1}{6} + \frac{7}{6}\sqrt{\frac{100}{N_0} } + \frac{1}{4} \right) \nonumber \\
    & \leq \frac{2^{-k}}{1-\gamma}. \label{eqn:q_k_induction_case_2}
\end{align}
By a union bound argument, we can conclude that the relation $\|Q^{(k)} - \starQ\|_{\infty} \leq \frac{2^{-k}}{1-\gamma}$ holds with probability at least $1- \delta$. \\

The only thing left to verify is that the inputs to the compressor are always bounded by $D_k$ during the $k^{\text{th}}$ epoch. The following lemma provides a bound on the input to the compressor during any run of the \RE routine.

\begin{lemma}
    Consider the \normalfont{\RE} routine described in Alg.~\ref{alg:refine_estimate}. For all $l \leq L$ and all agents $m$, the following bound holds with probability $1- \frac{\delta}{2K}$:
    \begin{align*}
        \|Q_{l -\frac{1}{2}}^{(m)} - Q_{l-1}\|_{\infty} \leq \eta\|\barQ- \starQH\|_{\infty}\left( \frac{7}{6} \cdot (1+\gamma)  + 2\gamma \right) + \frac{\eta D}{70}
    \end{align*}
    \label{lemma:compressor_input_bound}
\end{lemma}

For the $k^{\text{th}}$ epoch, the RHS is given as
\begin{align*}
    \eta\|Q^{(k-1)}- \starQ_{\cH_k}\|_{\infty}\left( \frac{7}{6} \cdot (1+\gamma)  + 2\gamma \right) + \frac{\eta D_k}{70} & \leq \frac{13}{3} \left(\|Q^{(k-1)}- \starQ\|_{\infty} + \|\starQ- \starQ_{\cH_k}\|_{\infty} \right) + \frac{ D_k}{70} \\
    & \leq \frac{13}{3} \cdot \frac{15}{14} \|Q^{(k-1)}- \starQ\|_{\infty}  + \frac{D_k}{70} \\
    & \leq \left(\frac{195}{42}  + \frac{8}{70}\right) \cdot \frac{2^{-(k-1)}}{1-\gamma} \\
    & \leq 8 \cdot \frac{2^{-(k-1)}}{1-\gamma} := D_k.
\end{align*}
In the third step, we used the same sequence of arguments as used in Eqns.~\eqref{eqn:q_k_induction_case_1} and~\eqref{eqn:q_k_induction_case_2} and the fourth step, we used the bound on $\|Q^{(k-1)}- \starQ\|_{\infty}$ from Eqn.~\eqref{eqn:q_k_relation} and the prescribed value of $D_k$.


% \subsection{Proof of Lemma}

% The proof of this lemma is inspired by analysis of the variance reduced Q-learning algorithm proposed in~\cite{Wainwright2019VarianceReduced}. Note that the update scheme of variance reduced learning resembles that of the classic Q-learning scheme, i.e., fixed-point iteration, with a different operator defined as follows:
% \begin{align}
%     \cH(Q) := \cT(Q) - \cT(\barQ) + \tildeT_N(\barQ).
% \end{align}
% The update scheme at step $l \geq 1$ in Eqn.~\eqref{} can then be written as
% \begin{align}
%     Q_l^{(m)} = (1-\eta) Q_{l-1} + \eta \widehat{\cH}_l^{(m)}(Q_{l-1}),
% \end{align}
% where $\widehat{\cH}_l^{(m)}(Q) := \hatT_l^{(m)}(Q) - \hatT_l^{(m)}(\barQ) + \tildeT_N(\barQ)$ is a stochastic, unbiased estimate of the operator $\cH$, similar to $\hatT_l^{(m)}(Q)$. Let $Q_{\cH}^{\star}$ denote the fixed point of $\cH$. Then the update scheme in Eqn.~\eqref{}, drives the sequence $\{Q_{l}\}_{l}$ to $Q_{\cH}^{\star}$. As long as $\|Q^{\star} - Q_{\cH}^{\star}\|_{\infty}$ is small, the required error $\|Q_l - Q^{\star}\|_{\infty}$ can also be controlled. We establish the relation in the lemma using an inductive approach. The base case holds immediately, by definition. Assume that the result holds for $l - 1$.


\subsection{Proof of Lemma~\ref{lemma:q_l_star_q_h_err}}

Let us begin with analyzing the evolution of the sequence $\{Q_l\}_{l= 1}^L$ during a run of the \RE routine. The sequence $\{Q_l\}_{l= 1}^L$ satisfies the following recursion:
\begin{align}
    Q_l & = Q_{l-1} + \frac{1}{M} \sum_{m = 1}^M \sC\left( Q_{l- \frac{1}{2}}^{(m)} - Q_{l-1}; D, J \right ) \nonumber \\
    & = Q_{l-1} + \frac{1}{M} \sum_{m = 1}^M \left( Q_{l- \frac{1}{2}}^{(m)} - Q_{l-1} + \zeta_l^{(m)} \right) \nonumber \\
    & = \frac{1}{M} \sum_{m = 1}^M \left( Q_{l- \frac{1}{2}}^{(m)} + \zeta_l^{(m)} \right) \nonumber \\
    & = (1-\eta)Q_{l-1} + \frac{\eta}{M} \sum_{m = 1}^M \hatH_l^{(m)}(Q_{l-1})  + \underbrace{\frac{1}{M} \sum_{m = 1}^M \zeta_l^{(m)}}_{ := \zeta_l }. \label{eqn:q_l_recursive_update}
\end{align}
In the above expression, $\zeta_l^{(m)}$ denotes the quantization noise introduced at agent $m$ in the $l^{\text{th}}$ update. By the construction of the compression routine described in Sec.~\ref{}, it is straightforward to note that $\zeta_l^{(m)}$ is a zero mean random vector whose coordinates are independent, $D^2 \cdot 4^{-J}$-sub-Gaussian random variables. Thus, $\zeta_l$ is also a zero mean random vector whose coordinates are independent, $\frac{D^2}{M \cdot 4^{J}}$-sub-Gaussian random variables. On subtracting $\starQH$ from both sides of Eqn.~\eqref{eqn:q_l_recursive_update}, we obtain
\begin{align}
    Q_l - \starQH & = (1-\eta)(Q_{l-1} - \starQH) + \frac{\eta}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(Q_{l-1}) - \starQH \right) + \zeta_l \nonumber \\
    & = (1-\eta)(Q_{l-1} - \starQH) + \frac{\eta}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(Q_{l-1}) - \hatH_l^{(m)}(\starQH) \right) + \frac{\eta}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(\starQH) - \cH(\starQH) \right) + \zeta_l. \label{eqn:q_l_minus_star_q_h}
\end{align}
Consequently, 
\begin{align}
    \|Q_l - \starQH\|_{\infty} & \leq (1-\eta)\|Q_{l-1} - \starQH\|_{\infty} + \frac{\eta}{M} \sum_{m = 1}^M \left\|\hatH_l^{(m)}(Q_{l-1}) - \hatH_l^{(m)}(\starQH) \right\|_{\infty} \nonumber \\
    & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ + \left\| \frac{\eta}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(\starQH) - \cH(\starQH) \right) \right\|_{\infty} + \left\|\zeta_l\right\|_{\infty} \nonumber \\
    & \leq (1-\eta)\|Q_{l-1} - \starQH\|_{\infty} + \frac{\eta\gamma}{M} \sum_{m = 1}^M \|Q_{l-1} - \starQH\|_{\infty} + \left\| \frac{\eta}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(\starQH) - \cH(\starQH) \right) \right\|_{\infty} + \left\|\zeta_l\right\|_{\infty} \nonumber \\
    & \leq (1-\eta(1-\gamma))\|Q_{l-1} - \starQH\|_{\infty}  + \eta \left\| \frac{1}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(\starQH) - \cH(\starQH) \right) \right\|_{\infty} + \left\|\zeta_l\right\|_{\infty}. \label{eqn:Q_l_recursion_inf_norm}
\end{align}
In the second step, we used the fact that
\begin{align*}
    \left\|\hatH_l^{(m)}(Q) - \hatH_l^{(m)}(\starQH)\right\|_{\infty} = \left\| \hatT_l^{(m)}(Q) - \hatT_l^{(m)}(\starQH) \right\|_{\infty} \leq \gamma \left\| Q - \starQH \right\|_{\infty},
\end{align*}
which holds for all $Q$ since $\hatT$ is a $\gamma$-contractive operator. For second term on the RHS, we have,
\begin{align*}
    \frac{1}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(\starQH) - \cH(\starQH) \right) = \frac{1}{MB} \sum_{m = 1}^M \sum_{z \in \cZ_l^{(m)}} \left(\cT_z(\starQH) - \cT_z(\barQ) - \cT(\starQH) + \cT(\barQ) \right).
\end{align*}
Note that $\cT_z(\starQH) - \cT_z(\barQ) - \cT(\starQH) + \cT(\barQ)$ is a zero mean random vector satisfying $\|\cT_z(\starQH) - \cT_z(\barQ) - \cT(\starQH) + \cT(\barQ)\|_{\infty} \leq 2\gamma \| \barQ - \starQH\|_{\infty}$. Thus, each coordinate is a $(2\gamma \| \barQ - \starQH\|_{\infty})^2$-sub-Gaussian vector. On using the tail bounds for a maximum of sub-Gaussian random variables, we obtain that 
\begin{align}
    \left\|\frac{1}{M} \sum_{m = 1}^M \left(\hatH_l^{(m)}(\starQH) - \cH(\starQH) \right) \right\|_{\infty} \leq 2\gamma \| \barQ - \starQH\|_{\infty} \cdot \sqrt{\frac{2}{MB} \log\left(\frac{8KL|\cS||\cA|}{\delta} \right)} \label{eqn:H_err_bound}
\end{align}
holds with probability at least $1 - \frac{\delta}{4KL}$. Similarly, we can also conclude that
\begin{align}
    \|\zeta_l\|_{\infty} \leq D \cdot 2^{-J} \cdot \sqrt{\frac{2}{M} \log\left(\frac{8KL|\cS||\cA|}{\delta} \right)} \label{eqn:zeta_err_bound}
\end{align}
holds with probability at least $1 - \frac{\delta}{4KL}$.
% Given the quantization routine, it is straightforward to note that $\zeta_l^{(m)}$ is a sub-Gaussian random variable with variance proxy $\eta^2\|\hatH_l^{(m)}(Q_{l-1}) - Q_{l-1}\|_{\infty}^2 \cdot 4^{-J} \leq \eta^2(1+ \gamma)^{2}\|Q_{l-1} - \starQH\|_{\infty}^{2} \cdot 4^{-J}$, as $\hatH_l^{(m)}$ is a $\gamma$-contractive operator. Thus, with probability $1 - \delta/2L$,   
% \begin{align}
%     \|\zeta_l\|_{\infty} \leq \eta(1+ \gamma)\|Q_{l-1} - \starQH\|_{\infty} \cdot 2^{-J} \cdot \sqrt{\frac{2}{M} \log\left(\frac{4L}{\delta} \right)} \leq \frac{\eta(1 - \gamma)}{2}\|Q_{l-1} - \starQH\|_{\infty}. \label{eqn:zeta_err_bound}
% \end{align}
% \blue{Need to choose $J$}.
On plugging the results from Eqns.~\eqref{eqn:H_err_bound} and~\eqref{eqn:zeta_err_bound} into Eqn.~\eqref{eqn:Q_l_recursion_inf_norm} and letting $\kappa := \log\left(\frac{8KL|\cS||\cA|}{\delta} \right)$, we obtain that the following relation holds with probability $1- \frac{\delta}{2KL}$:
\begin{align*}
    \|Q_l - \starQH\|_{\infty} & \leq (1-\eta(1-\gamma))\|Q_{l-1} - \starQH\|_{\infty}  + 2\eta \gamma \| \barQ - \starQH\|_{\infty} \cdot \sqrt{\frac{2\kappa}{MB}}  + D \cdot 2^{-J} \cdot \sqrt{\frac{2\kappa}{M}}. 
\end{align*}
Unrolling the above recursion yields the following relation which holds with probability $1 - \frac{\delta}{2K}$:
% Upon unrolling in the recursion in Eqn.~\eqref{eqn:Q_l_recursion_inf_norm} and using the results from Eqns.~\eqref{eqn:H_err_bound} and~\eqref{eqn:zeta_err_bound}, we obtain,
\begin{align}
    \|Q_L - \starQH\|_{\infty} & \leq \left(1-\eta(1-\gamma)\right)^{L}\|Q_{0} - \starQH\|_{\infty}  +   \sqrt{\frac{2\kappa}{M}} \left(\frac{2\eta \gamma}{\sqrt{B}} \| \barQ - \starQH\|_{\infty}  + D \cdot 2^{-J} \right) \cdot \sum_{l = 1}^{L} \left(1-\eta(1-\gamma)\right)^{L - l} \nonumber\\
    & \leq \left(1-\eta(1-\gamma)\right)^{L}\|\barQ - \starQH\|_{\infty}  +  \frac{1}{\eta(1-\gamma)} \sqrt{\frac{2\kappa}{M}} \left(\frac{2\eta \gamma}{\sqrt{B}} \| \barQ - \starQH\|_{\infty}  + D \cdot 2^{-J} \right)  \nonumber\\
    & \leq \|\barQ - \starQH\|_{\infty} \left(\left(1-\eta(1-\gamma)\right)^{L} + \frac{2 \gamma}{(1-\gamma)}\sqrt{\frac{2\kappa}{MB}} \right)  +  \frac{D \cdot 2^{-J}}{\eta(1-\gamma)} \cdot \sqrt{\frac{2\kappa}{M}}   \label{eqn:Q_L_inf_norm_orig_bound_step_3}\\
    % & \leq \left(1-\frac{\eta(1-\gamma)}{2}\right)^{L}\|Q_{0} - \starQH\|_{\infty}  +   \frac{4}{\eta(1-\gamma)} \cdot \| \barQ - \starQH\|_{\infty} \cdot \sqrt{\frac{2}{MB} \log\left(\frac{4L}{\delta} \right)} \nonumber \\
    % & \leq \| \barQ - \starQH\|_{\infty} \cdot \left[\left(1-\frac{\eta(1-\gamma)}{2}\right)^{L}  +   \frac{4}{\eta(1-\gamma)} \cdot \sqrt{\frac{2}{MB} \log\left(\frac{4L}{\delta} \right)}\right] \nonumber \\ 
    & \leq \frac{\|\barQ - \starQH\|_{\infty}}{6} + \frac{D}{70} \nonumber \\
    & \leq \frac{1}{6} \left(\| \barQ - \starQ\|_{\infty} + \| \starQ - \starQH\|_{\infty} \right) + \frac{D}{70}.
    \label{eqn:Q_L_inf_norm_orig_bound}
\end{align} 
The fourth step is obtained by plugging in the prescribed values of $B, L$ and $J$.


\subsection{Proof of Lemma~\ref{lemma:star_q_h_star_q_err}}

Intuitively, the error $\|\starQH - \starQ\|_{\infty}$ depends on the error term $\tildeT_N(\barQ) - \cT(\barQ)$. If the latter is small, then $\cH(Q)$ is close to $\cT(Q)$ and consequently so are $\starQH$ and $\starQ$. Thus, we begin with bounding the term $\tildeT_N(\barQ) - \cT(\barQ)$. 
% The proof of Lemma xxx is based on the result in Lemma $4$ of~\cite{Wainwright2019VarianceReduced}. To invoke that result, we first obtain a bound on $\tildeT_N(\barQ) - \cT(\barQ)$. 
We have,
\begin{align}
    \tildeT_N(\barQ) - \cT(\barQ) & = \overline{Q} + \frac{1}{M} \sum_{m = 1}^M \sC\left( \tildeT^{(m)}_N(\overline{Q}) - \barQ \right) - \cT(\barQ) \nonumber \\
    & =\frac{1}{M} \sum_{m = 1}^M \left( \tildeT^{(m)}_N(\overline{Q}) + \tilde{\zeta}_N^{(m)} \right)  - \cT(\barQ) \nonumber  \\
     & =\frac{1}{M} \sum_{m = 1}^M \left( \tildeT^{(m)}_N(\overline{Q}) - \tildeT^{(m)}_N(\starQ) - \cT(\barQ) + \cT(\starQ) \right)   + \frac{1}{M} \sum_{m = 1}^M \tilde{\zeta}_N^{(m)} +  \frac{1}{M} \sum_{m = 1}^M \left( \tildeT^{(m)}_N(\starQ) -  \cT(\starQ) \right), \label{eqn:tilde_T_N_err_total}
\end{align}
where once again $\tilde{\zeta}_N^{(m)}$ denotes the quantization error at agent $m$.
Similar to Eqns.~\eqref{eqn:H_err_bound} and~\eqref{eqn:zeta_err_bound}, we can conclude that each of the following relations hold with probability $1 - \frac{\delta}{6K}$.
\begin{align}
    \left\|\frac{1}{M} \sum_{m = 1}^M \left( \tildeT^{(m)}_N(\overline{Q}) - \tildeT^{(m)}_N(\starQ) - \cT(\barQ) + \cT(\starQ) \right)\right\|_{\infty} \leq 2\gamma \| \barQ - \starQ\|_{\infty} \cdot \sqrt{\frac{2}{N} \log\left(\frac{12K|\cS||\cA|}{\delta} \right)}, \label{eqn:tilde_T_N_err_term_1}
\end{align}
\begin{align}
    \left\|\frac{1}{M} \sum_{m = 1}^M \tilde{\zeta}_N^{(m)}\right\|_{\infty} \leq D \cdot 2^{-J} \cdot \sqrt{\frac{2}{M} \log\left(\frac{12K|\cS||\cA|}{\delta} \right)}
    % (1+ \gamma)\|\barQ - \starQ\|_{\infty} \cdot 2^{-J} \cdot \sqrt{\frac{2}{M} \log\left(\frac{2}{\delta} \right)} \leq \frac{(1 - \gamma)}{C_0} \cdot \|\barQ - \starQ\|_{\infty}, 
    \label{eqn:tilde_T_N_err_term_2}
\end{align}
For the third term, we can rewrite it as
\begin{align*}
    \frac{1}{M} \sum_{m = 1}^M \left( \tildeT^{(m)}_N(\starQ) -  \cT(\starQ) \right) = \frac{1}{M \lceil N/M \rceil} \sum_{m = 1}^M \sum_{i = 1}^{\lceil N/M \rceil} \left( \cT_{Z_i^{(m)}}(\starQ) -  \cT(\starQ) \right).
\end{align*}
We will use Bernstein inequality element wise to bound the above term. Let $\bfsigma^{\star} \in \R^{|\cS| \times |\cA|}$ be such that $[\bfsigma^{\star}(s,a)]^2 = \var(\cT_{Z}(\starQ)(s,a))$, i.e., $(s,a)^{\text{th}}$ element of $\bfsigma$ denotes the standard deviation of the random variable $\cT_{Z}(\starQ)(s,a)$. Since $\|\cT_{Z}(\starQ) -  \cT(\starQ)\|_{\infty} \leq \frac{1}{1-\gamma}$ a.s., Bernstein inequality gives us that
\begin{align}
    \left|\frac{1}{M} \sum_{m = 1}^M \left( \tildeT^{(m)}_N(\starQ)(s,a) -  \cT(\starQ)(s,a) \right) \right| \leq \bfsigma^{\star}(s,a) \sqrt{\frac{2}{N}\log\left(\frac{6K|\cS||\cA|}{\delta} \right)} + \frac{2}{3N(1- \gamma)} \log\left(\frac{6K|\cS||\cA|}{\delta} \right). \label{eqn:tilde_T_N_err_term_3}
\end{align}
holds simultaneously for all $(s,a) \in \cS \times \cA$ with probability at least $1 - \frac{\delta}{6K}$. 
% Recall that for vectors we use $\leq$ to denote an element wise relation. 
On combining Eqns.~\eqref{eqn:tilde_T_N_err_total},~\eqref{eqn:tilde_T_N_err_term_1},~\eqref{eqn:tilde_T_N_err_term_2} and~\eqref{eqn:tilde_T_N_err_term_3}, we obtain that 
\begin{align}
    \left|\tildeT_N(\barQ)(s,a) - \cT(\barQ)(s,a) \right| & =\| \barQ - \starQ\|_{\infty}  \cdot \sqrt{\frac{8\kappa'}{N} } + \bfsigma^{\star}(s,a) \sqrt{\frac{2\kappa'}{N}} + \frac{2\kappa'}{3N(1- \gamma)} + D \cdot 2^{-J} \cdot \sqrt{\frac{2\kappa'}{M}},  \label{eqn:tilde_T_N_err_final_bound}
     % \left(   + \frac{(1 - \gamma)}{C_0} \right) \bfone   +  \sigma^{\star} \sqrt{\frac{2}{N}\log\left(\frac{1}{\delta} \right)} + \frac{2}{3N(1- \gamma)} \log\left(\frac{1}{\delta} \right) \bfone
\end{align}
holds simultaneously for all $(s,a) \in \cS \times \cA$ with probability at least $1 - \frac{\delta}{2K}$, where $\kappa' = \log\left(\frac{12K|\cS||\cA|}{\delta} \right)$. Using the result from~\citep[Lemma 4]{Wainwright2019VarianceReduced} along with Eqn.~\eqref{eqn:tilde_T_N_err_final_bound}, we can conclude that
\begin{align}
    \|\starQH - \starQ\|_{\infty} & \leq \| \barQ - \starQ\|_{\infty} \cdot \sqrt{\frac{8\kappa'}{N(1-\gamma)^2} } +  \sqrt{\frac{32\kappa'}{N(1-\gamma)^3}} + \frac{2\kappa'}{3N(1- \gamma)^2} + \frac{D \cdot 2^{-J}}{(1-\gamma)} \cdot \sqrt{\frac{2\kappa'}{M}} \nonumber \\
    & \leq \| \barQ - \starQ\|_{\infty} \cdot \sqrt{\frac{8\kappa'}{N(1-\gamma)^2} } +  \sqrt{\frac{32\kappa'}{N(1-\gamma)^3}} + \frac{2\kappa'}{3N(1- \gamma)^2} + \frac{D}{40},
    % \left(\sqrt{\frac{18}{N(1-\gamma)^2} \log\left(\frac{2}{\delta} \right)}   + \frac{1}{C_0} \right)    +  \sqrt{\frac{32}{N(1-\gamma)^3}\log\left(\frac{1}{\delta} \right)} + \frac{2}{3N(1- \gamma)^2} \log\left(\frac{1}{\delta} \right). 
    \label{eqn:Q_H_Q_star_error_bound}
\end{align}
where once again we use the value of $J$ in the last step.

% On combining the bounds in Eqns.~\eqref{eqn:Q_L_inf_norm_orig_bound} and~\eqref{eqn:Q_H_Q_star_error_bound}, we can conclude that 
% \begin{align}
%      \|Q_L - \starQ\|_{\infty}  & \leq  \|Q_L - \starQH\|_{\infty} + \| \starQ - \starQH\|_{\infty} \nonumber \\
%     & \leq \frac{1}{4} \left(\| \barQ - \starQ\|_{\infty} + 5 \| \starQ - \starQH\|_{\infty} \right) \nonumber \\
%     & \leq \frac{1}{4} \cdot \| \barQ - \starQ\|_{\infty} \cdot \left(1 + \sqrt{\frac{450}{N(1-\gamma)^2} \log\left(\frac{2}{\delta} \right)}   + \frac{5}{C_0} \right)    +  \sqrt{\frac{50}{N(1-\gamma)^3}\log\left(\frac{1}{\delta} \right)} + \frac{5}{6N(1- \gamma)^2} \log\left(\frac{1}{\delta} \right).
% \end{align}

\subsection{Proof of Lemma~\ref{lemma:compressor_input_bound}}

From the iterate update rule in Eqn.~\eqref{eqn:q_l_update_rule_with_h}, for any agent $m$ we have,
\begin{align*}
    Q_{l - \frac{1}{2}}^{(m)} - Q_{l-1} & = \eta(\hatH_{l-1}^{(m)}(Q_{l-1}) - Q_{l-1}) \\
    & = \eta(\hatH_{l-1}^{(m)}(Q_{l-1}) - \hatH_{l-1}^{(m)}(\starQH) + \hatH_{l-1}^{(m)}(\starQH) - \cH(\starQH) + \starQH - Q_{l-1}).
\end{align*}
Thus,
\begin{align*}
    \|Q_{l - \frac{1}{2}}^{(m)} - Q_{l-1}\|_{\infty} & \leq \eta\left( \|\hatH_{l-1}^{(m)}(Q_{l-1}) - \hatH_{l-1}^{(m)}(\starQH)\|_{\infty} + \|\hatH_{l-1}^{(m)}(\starQH) - \cH(\starQH)\|_{\infty} + \|\starQH - Q_{l-1}\|_{\infty}\right) \\
    & \leq \eta\left( \gamma \|Q_{l-1} - \starQH\|_{\infty} + 2\gamma\|\barQ- \starQH\|_{\infty} + \|\starQH - Q_{l-1}\|_{\infty}\right) \\
    & \leq \eta\left( (1+\gamma) \|Q_{l-1} - \starQH\|_{\infty} + 2\gamma\|\barQ- \starQH\|_{\infty} \right) \\
    & \leq \eta\|\barQ- \starQH\|_{\infty}\left( \frac{7}{6} \cdot (1+\gamma)  + 2\gamma \right) + \frac{\eta D}{70},
\end{align*}
holds with probability $1- \frac{\delta}{2KL}$. The last step in the above relation follows from Eqn.~\eqref{eqn:Q_L_inf_norm_orig_bound_step_3} evaluated at a general value of $l$ and the prescribed value of $J$. By a union bound argument, the above relation holds for all $l$ with probability at least $1- \frac{\delta}{2K}$.
